Online Interactive Collaborative Filtering Using Multi-Armed Bandit with Dependent Arms

Online interactive recommender systems strive to promptly suggest to consumers appropriate items (e.g., movies, news articles) according to the current context including both the consumer and item content information. However, such context information is often unavailable in practice for the recommendation, where only the users' interaction data on items can be utilized. Moreover, the lack of interaction records, especially for new users and items, worsens the performance of recommendation further. To address these issues, collaborative filtering (CF), one of the recommendation techniques relying on the interaction data only, as well as the online multi-armed bandit mechanisms, capable of achieving the balance between exploitation and exploration, are adopted in the online interactive recommendation settings, by assuming independent items (i.e., arms). Nonetheless, the assumption rarely holds in reality, since the real-world items tend to be correlated with each other (e.g., two articles with similar topics). In this paper, we study online interactive collaborative filtering problems by considering the dependencies among items. We explicitly formulate the item dependencies as the clusters on arms, where the arms within a single cluster share the similar latent topics. In light of the topic modeling techniques, we come up with a generative model to generate the items from their underlying topics. Furthermore, an efficient online algorithm based on particle learning is developed for inferring both latent parameters and states of our model. Additionally, our inferred model can be naturally integrated with existing multi-armed selection strategies in the online interactive collaborating setting. Empirical studies on two real-world applications, online recommendations of movies and news, demonstrate both the effectiveness and efficiency of the proposed approach.

==> algorithm.tex <==
\section{Algorithm}

\subsection{Re-sample Particles with Weights}
\begin{equation}
 \begin{split}
    weight \propto \{ MVST_{(2\cdot\alpha)}[y_{m,t}| \mathbf{p}_m \mathbf{\mu}_{\mathbf{q}_{n(t)}}, \frac{\alpha}{\beta}(\mathbf{I}+{\mathbf{p}_m^{\intercal}}\mathbf{\Sigma}_{\mathbf{q}_{n(t)}}\mathbf{p}_m)] \\ E({\Phi_{k,n(t)}})  \}
 \end{split}
 \label{eq:weight}
 \end{equation}


\subsection{Latent State Inference}

\begin{equation}
 \begin{split}
 S_{t}^{\Phi_{k,n}} = \frac{\mathcal{I}(X_{m,t}=n)r_{m,t} + \eta_{k,n}}{\sum_{n=1}^{N}[\mathcal{I}(X_{m,t}=n)r_{m,t} + \eta_{k,n}]}
 \end{split}
 \end{equation}

\begin{equation}
 \begin{split}
 S_{t}^{\mathbf{p}_{m,k}} = \frac{\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}}{\sum_{k=1}^{K}[\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}]}
 \end{split}
 \end{equation}

\begin{equation}
 \begin{split}
 P(z_{m,t}|S_{t}^{\Phi_{k,n}}, S_{t}^{p_{m,k}}) = S_{t}^{\Phi_{k,n}} \cdot S_{t}^{p_{m,k}}
 \end{split}
 \end{equation}

\subsection{Parameter Statistics Inference}

\begin{equation}
 \begin{split}
 \mathbf{\mu}_{\mathbf{q}_n}^{*} = (\mathbf{\Sigma}_{\mathbf{q}_n}^{-1} + \mathbf{p}_m^{T}\mathbf{p}_m)^{-1}(\mathbf{\Sigma}_{\mathbf{q}_n}^{-1}\mathbf{\mu}_{\mathbf{q}_n} + \mathbf{p}_m^{T}r_{m,t})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
 \mathbf{\Sigma}_{\mathbf{q}_n}^{*} = (\mathbf{\Sigma}_{\mathbf{q}_n}^{-1} + \mathbf{p}_m^{T}\mathbf{p}_m)^{-1}
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
 \alpha^{*} = \alpha + \frac{1}{2}
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
 \beta^{*} = \beta + \frac{1}{2}(\mathbf{\mu}_{\mathbf{q}_n}^{T} \mathbf{\Sigma}_{\mathbf{q}_n}^{-1} \mathbf{\mu}_{\mathbf{q}_n} +
 r_{m,t}^{T}r_{m,t} - \mathbf{\mu}_{\mathbf{q}_n}^{*^{T}} \mathbf{\Sigma}_{\mathbf{q}_n}^{*^{-1}} \mathbf{\mu}_{\mathbf{q}_n}^{*}
 )
 \end{split}
 \end{equation}

 \begin{equation}
   \begin{split}
     \eta^{*}_{k,n} = \mathcal{I}(X_{m,t}=n)r_{m,t} + \eta_{k,n}
   \end{split}
 \end{equation}

 \begin{equation}
   \begin{split}
     \lambda^{*}_{k} = \mathcal{I}(Z_{m,t}=k)r_{m,t} + \lambda_{k}
   \end{split}
 \end{equation}


\subsection{Parameter Inference}

 \begin{equation}
 \begin{split}
  \mathbf{p}_{m,k} \sim P(\mathbf{p}_m | S_{t}^{\mathbf{p}_{m,k}})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
  \Phi_{k,n} \sim P(\Phi_{k,n}| S_{t}^{\Phi_{k,n}})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
  \mathbf{q}_n \sim \mathcal{N}(\mathbf{\mu}_{\mathbf{q}_n}^{*}, \sigma_n \mathbf{\Sigma}_{\mathbf{q}_n}^{*})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
  \sigma_n \sim \mathcal{IG}(\alpha^{*}, \beta^{*})
 \end{split}
 \end{equation}


==> arXiv copy/abstract.tex <==
Online interactive recommender systems strive to promptly suggest to consumers appropriate items (e.g., movies, news articles) according to the current context including both the consumer and item content information. %, and try to continuously maximize the consumers' satisfaction in a long run.
However, such context information is often unavailable in practice for the recommendation, where only the users' interaction data on items can be utilized.
%However, the content information for both users and items is often unavailable in practice for the recommendation, excluding the users' interaction data on items. Furthermore,
Moreover, the lack of interaction records, especially for new users and items, worsens the performance of recommendation further. To address these issues, collaborative filtering (CF), one of the recommendation techniques relying on the interaction data only, as well as the online multi-armed bandit mechanisms, capable of achieving the balance between exploitation and exploration, are adopted in the online interactive recommendation settings, by assuming independent items (i.e., arms). Nonetheless, the assumption rarely holds in reality, since the real-world items tend to be correlated with each other (e.g., two articles with similar topics).

In this paper, we study online interactive collaborative filtering problems by considering the dependencies among items. We explicitly formulate the item dependencies as the clusters on arms, where the arms within a single cluster share the similar latent topics.
In light of the topic modeling techniques, we come up with a generative model to generate the items from their underlying topics. 
Furthermore, an efficient online algorithm based on particle learning is developed for inferring both latent parameters and states of our model. 
Additionally, our inferred model can be naturally integrated with existing multi-armed selection strategies in the online interactive collaborating setting. Empirical studies on two real-world applications, online recommendations of movies and news, demonstrate both the effectiveness and efficiency of the proposed approach.

\begin{comment}

To infer the our model from the online interaction data,

in practice, only the interaction data between users and items can be utilized for recommendation, since the content information for both users and items are often unavailable due to privacy or sampling constraints. Even if the recomm

 in practice. Moreover, the rec

the recommender system usually suffers ineffective performance due to the unavailability of information. Collaborative filtering (CF), one of the recommendation techniques only relying on users' feedbacks on items, has gained its popularity since the content information for both users and items are often unavailable in practice.

The overwhelming amount of data necessitates the efficient online interactive recommendation system where the online users constantly interact with the system, and the users' feedbacks are instantly acquired for further users' preferences tracking as well as recommendation performance improvement. However,

%It is demanding to enable recommender systems an online behavior in which an item is sequentially recommended to a user and the up-to-date feedback from the user.
Collaborative filtering (CF), one of the recommendation techniques only relying on users' feedbacks on items, has gained its popularity since the content information for both users and items are often unavailable in practice. However, cold start problem is In this paper, we formulate the online recommendation problem as a multi-armed bandit problem

 Collaborative filtering (CF), one of those recommender systems that utilize only users' feedback on items, is typically formulated as a matrix factorization (MF) problem. It is demanding to enable recommender systems an online behavior in which an item is sequentially recommended to a user and the up-to-date feedback from the user is instantly applied for refining the recommender system because it empowers the system the efficiency and capability to adapt over time. This usually requires not only sequential online inference techniques such as particle learning to update the model but also techniques like multi-armed bandit to address the cold-start problem since users have insufficient ratings on items at the very beginning of training the system.

However, the existing prior work on recommender systems with the multi-armed bandit techniques all assumes that the success probabilities of pulling the arms i.e., recommending the items are independent, which is rarely holding in practice.

In this paper, we propose an online MF-based recommender system that exploits dependency among arms by integrating topic modeling to soft cluster the arms and share feedbacks within clusters. We conduct extensive experiments for our proposed algorithms on two real-world datasets Yahoo! Today News and MovieLens (10M). Results demonstrate the effectiveness and efficiency of our approaches over the current state-of-arts and the capability of more efficiently utilizing feedbacks among dependent arms.
\end{comment}



==> arXiv copy/algorithm.tex <==
\section{Algorithm}

\subsection{Re-sample Particles with Weights}
\begin{equation}
 \begin{split}
    weight \propto \{ MVST_{(2\cdot\alpha)}[y_{m,t}| \mathbf{p}_m \mathbf{\mu}_{\mathbf{q}_{n(t)}}, \frac{\alpha}{\beta}(\mathbf{I}+{\mathbf{p}_m^{\intercal}}\mathbf{\Sigma}_{\mathbf{q}_{n(t)}}\mathbf{p}_m)] \\ E({\Phi_{k,n(t)}})  \}
 \end{split}
 \label{eq:weight}
 \end{equation}


\subsection{Latent State Inference}

\begin{equation}
 \begin{split}
 S_{t}^{\Phi_{k,n}} = \frac{\mathcal{I}(X_{m,t}=n)r_{m,t} + \eta_{k,n}}{\sum_{n=1}^{N}[\mathcal{I}(X_{m,t}=n)r_{m,t} + \eta_{k,n}]}
 \end{split}
 \end{equation}

\begin{equation}
 \begin{split}
 S_{t}^{\mathbf{p}_{m,k}} = \frac{\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}}{\sum_{k=1}^{K}[\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}]}
 \end{split}
 \end{equation}

\begin{equation}
 \begin{split}
 P(z_{m,t}|S_{t}^{\Phi_{k,n}}, S_{t}^{p_{m,k}}) = S_{t}^{\Phi_{k,n}} \cdot S_{t}^{p_{m,k}}
 \end{split}
 \end{equation}

\subsection{Parameter Statistics Inference}

\begin{equation}
 \begin{split}
 \mathbf{\mu}_{\mathbf{q}_n}^{*} = (\mathbf{\Sigma}_{\mathbf{q}_n}^{-1} + \mathbf{p}_m^{T}\mathbf{p}_m)^{-1}(\mathbf{\Sigma}_{\mathbf{q}_n}^{-1}\mathbf{\mu}_{\mathbf{q}_n} + \mathbf{p}_m^{T}r_{m,t})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
 \mathbf{\Sigma}_{\mathbf{q}_n}^{*} = (\mathbf{\Sigma}_{\mathbf{q}_n}^{-1} + \mathbf{p}_m^{T}\mathbf{p}_m)^{-1}
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
 \alpha^{*} = \alpha + \frac{1}{2}
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
 \beta^{*} = \beta + \frac{1}{2}(\mathbf{\mu}_{\mathbf{q}_n}^{T} \mathbf{\Sigma}_{\mathbf{q}_n}^{-1} \mathbf{\mu}_{\mathbf{q}_n} +
 r_{m,t}^{T}r_{m,t} - \mathbf{\mu}_{\mathbf{q}_n}^{*^{T}} \mathbf{\Sigma}_{\mathbf{q}_n}^{*^{-1}} \mathbf{\mu}_{\mathbf{q}_n}^{*}
 )
 \end{split}
 \end{equation}

 \begin{equation}
   \begin{split}
     \eta^{*}_{k,n} = \mathcal{I}(X_{m,t}=n)r_{m,t} + \eta_{k,n}
   \end{split}
 \end{equation}

 \begin{equation}
   \begin{split}
     \lambda^{*}_{k} = \mathcal{I}(Z_{m,t}=k)r_{m,t} + \lambda_{k}
   \end{split}
 \end{equation}


\subsection{Parameter Inference}

 \begin{equation}
 \begin{split}
  \mathbf{p}_{m,k} \sim P(\mathbf{p}_m | S_{t}^{\mathbf{p}_{m,k}})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
  \Phi_{k,n} \sim P(\Phi_{k,n}| S_{t}^{\Phi_{k,n}})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
  \mathbf{q}_n \sim \mathcal{N}(\mathbf{\mu}_{\mathbf{q}_n}^{*}, \sigma_n \mathbf{\Sigma}_{\mathbf{q}_n}^{*})
 \end{split}
 \end{equation}

 \begin{equation}
 \begin{split}
  \sigma_n \sim \mathcal{IG}(\alpha^{*}, \beta^{*})
 \end{split}
 \end{equation}


==> arXiv copy/conclusion-future-work.tex <==
\section{Conclusion and Future Work} \label{sec:conclusion}

In this paper, we propose an interactive collaborative topic regression model that adopts a generative process based on topic modeling to explicitly formulate the arm dependencies as the clusters on arms, where dependent arms are assumed to be generated from the same cluster. Every time an arm is pulled, the feedback is not only used for inferring the involved user and item latent vectors, but also employed to update the latent parameters with respect to the arm's cluster. The latent cluster parameters further help with the reward prediction for other arms in the same cluster. We conduct empirical studies on two real-world applications, including movie and news recommendation, and the experimental results demonstrate the effectiveness of our proposed approach.

\noindent \ \ \ \ Individual preferences on news and movies usually evolve over time. One possible research direction is to extend our model considering the time-varying property in user preferences for better online personal recommendation~\cite{zeng2016online}. In this paper, we formulate the arm dependencis as soft clustering. Another possible research direction is to explicitly eplore the hirerarchial structure among arms~\cite{zeng2017knowledge} (i.e. items in specific domain areas), which can be manually or dynamically constructed using domain knowledge~\cite{wang2017constructing}.


==> arXiv copy/experiment.tex <==
\section{Empirical Study}\label{sec:experiment}

  To demonstrate the efficiency of our proposed algorithm, we conduct our experimental study over two popular real-world dataset: Yahoo! Today News and MovieLens (10M).
First, we outline the general implementation of the baseline algorithms for comparison. Second,  we start with a brief description of the data sets and evaluation method.
Finally, we show and discuss the comparative experimental results of both the proposed algorithms and the baseline algorithms, and a case study on movie topic distribution analysis of MovieLens (10M).

\subsection{Baseline Algorithms}\label{sec:baseline}
In the experiment, we demonstrate the performance of our methods by comparing them with the following baseline algorithms:

\begin{enumerate}
  \item \texttt{Random}: it randomly selects an item recommending to the target user.

  \item \texttt{$\epsilon$-greedy}($\epsilon$): it randomly selects an item with probability $\epsilon$ and selects the item of the largest predicted reward with probability $1-\epsilon$, where $\epsilon$ is a predefined parameter.
      %When $\epsilon = 0$, it is equivalent to the \texttt{Exploit} policy.

  \item \texttt{UCB}($\lambda$): it picks the item $j(t)$ with the highest rewards at time $t$ as follows:
  \begin{equation*}
     j(t) = \arg\max_{j=1,\dots,N}(\hat{\mu_i} + \lambda\sqrt{\frac{2ln(t)}{n_{i(t)}}})
%  \vspace{-0.10in}
  \end{equation*}
  where $n_{i(t)}$ is the number of times that item $n_i$ has been recommended until time $t$.
  %When $\lambda = 0$, it becomes the \texttt{Exploit} policy that has no exploration.
  \item \texttt{TS}($S_i(t), F_i(t)$): Thompson sampling described in Section~\ref{subsec:base}, randomly draws the expected reward from the Beta posterior distribution, and selects the item of the largest predicted reward. $S_i(t)$/$F_i(t)$ indicates the number of positive/negative feedback on item $i$ until time $t$.
  \item \texttt{PTS}($d$, $p$): Particle Thompson sampling for matrix factorization, approximates the posterior of the latent feature vectors by updating a set of particles. Here $d$ is the dimension of latent feature vector and $p$ is the number of particles.
  %\item \texttt{ICTR}(\#k, \#particles): Interactive collaborative topic regression integrates our proposed interactive collaborative topic regression model with \texttt{TS} bandit algorithm. \#k indicates the dimension of latent feature vector and the number of the topics, while \#particles represents the number of particles.
\end{enumerate}

 Our methods proposed in this paper include:
 \begin{enumerate}
 	\item \texttt{ICTRTS}($d$, $p$): it denotes our proposed interactive collaborative topic regression model with \texttt{TS} bandit algorithm. Here $d$ is the dimension of latent feature vector and $p$ is the number of particles.
 	\item \texttt{ICTRUCB}($d$, $p$, $\gamma$): it indicates our proposed model with \texttt{UCB} bandit algorithm. Similar to \texttt{UCB}, $\gamma$ is given. Here $d$ is the dimension of latent feature vector and $p$ represents the number of particles.
 \end{enumerate}
\subsection{Datasets Description}
 We use two real-world datasets shown in Table~\ref{tab:datasets} to evaluate our proposed algorithms.
\begin{comment}
\begin{table}[!htb]
		\small
        \centering
        \caption{Description of Datasets.}
        \vspace{-0.1in}
        \scalebox{0.9}{
        \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Dataset}  & {\textbf{Yahoo News}}  & {\textbf{MovieLens (10M)}} & {\textbf{Netflix Prize}}\\
        \hline
        \texttt{\#users}   & 226,710    &  71,567    & 480,189   \\
        \hline
        \texttt{\#items}   & 652        &  10,681     &  17,770\\
       \hline
        \texttt{\#ratings} & 28,041,0150  &  10,000,054  &  100,480,507\\
       \hline
        \end{tabular}
        }
        \label{tab:datasets}
\vspace{-0.1in}
\end{table}
\end{comment}
\begin{table}[!htb]
        \centering
        \vspace{-0.1in}
        \caption{Description of Datasets.}
       
        \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Dataset}  & {\textbf{Yahoo News}}  & {\textbf{MovieLens (10M)}}\\
        \hline
        \texttt{\#users}   & 226,710    &  71,567       \\
        \hline
        \texttt{\#items}   & 652        &  10,681  \\
       \hline
        \texttt{\#ratings} & 28,041,0150  &  10,000,054  \\
       \hline
        \end{tabular}
        
        \label{tab:datasets}
\end{table}

\textbf{Yahoo! Today News:} The core task of personalized news recommendation is to display appropriate news articles on the web page for the users according to the potential interests of individuals. The recommender system often takes the instant feedback from users into account to improve the prediction of the potential interests of individuals, where the user feedback is about whether the users click the recommended article or not.
 %Additionally, every news article does not receive any feedbacks unless the news article is displayed to the user.
 Here, we formulate the personalized news recommendation problem as an instance of bandit problem, where each item corresponds to a news article and user information is considered as the identification of one user. The experimental data set is a collection based on a sample of anonymized user interaction on the news feeds, collected by the Yahoo! Today module and published by Yahoo! Research Lab\footnote{http://webscope.sandbox.yahoo.com/catalog.php}.
 %The dataset contains 28,041,015 visit events of user-news item interaction data.
 The dataset contains 15 days' visit events of user-news item interaction data. Besides, user's information, e.g., demographic information (age and gender), is provided for each visit event, and represented as the user identification.
 %Besides, the interaction data is also stamped with the user's local time, which is suitable for recommendation and temporal data mining.
 This data set has been used for evaluating contextual bandit algorithms in~\cite{li2010contextual}, \cite{li2012unbiased},\cite{tang2015personalized},\cite{zeng2016online}.
In our experiments, the visit events of the first day are utilized for selecting proper parameters of ICTR model, while 2.0 million of the remaining are used for the validation.
Each interactive record has a user ID, a news ID, the value of rating, the news pool and time stamp.

\textbf{MovieLens (10M):} Online movie recommender service aims to maximize the customer's satisfaction by recommending the proper movies to the target users according to their preference.
Specifically,
%an enormous amount of new movies will be brought into the movie pool.
several movies out of a movie pool are first displayed to users, and then users' feedback on displayed movies is collected for improving the user satisfaction.
Thereby, the problem of movie recommendation can be regarded as an instance of bandit problem in which an arm is a movie, a pull is regarded as a movie selection, and the reward indicates the feedbacks of user's rating on movies.
In our experiments, each rating associates a user ID, a movie ID, and a time stamp.
In order to use the \emph{replayer} evaluation method, each value of a rating is processed to be 1.0 if the rating is larger than 4.0/5.0 and 0.0 otherwise.
Additionally, top-N $(N=100)$ popular movies are selected as the movie pool.
\begin{comment}
\begin{figure}[htp!]
\centering
\begin{subfigure}{0.23\textwidth}
  \centering
  \scalebox{0.22}{
   \includegraphics{fig/10m-topItemIdList.eps}
  }
\caption{MovieLens (10M).}
\label{fig:10m-topItemIdList}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
  \centering
  \scalebox{0.22}{
   \includegraphics{fig/netflix-topItemIdList.eps}
  }
\caption{Netflix Prize.}
\label{fig:netflix-topItemIdList}
\end{subfigure}
\vspace{-0.1in}
\caption{Proportion of top-N itemId Pool.}
\label{fig:topItem-distribution}
\end{figure}
\end{comment}

\subsubsection{Evaluation Method}
We apply the \emph{replayer} method to evaluate our proposal method on the aforementioned two datasets.
 %since the number of items in the pool is not larger than $50$.
The \emph{replayer} method is first introduced in \cite{li2012unbiased}, which provides an unbiased offline evaluation via the historical logs. The main idea of \emph{replayer} is to replay each user visit to the algorithm under evaluation. If the recommended item by the testing algorithm is identical to the one in the historical log, this visit is considered as an impression of this item to the user. The ratio between the number of user clicks and the number of impressions is referred to as CTR. The work in \cite{li2012unbiased} shows that the CTR estimated by the \emph{replayer} method approaches the real CTR of the deployed online system.
%if the items in historical user visits are randomly recommended.

\subsubsection{CTR/Rating Optimization for News/Movies Recommendation}
In this section we first conduct the performance evaluation for each algorithm with different parameter settings. All baseline algorithms are configured with their best parameter settings provided by Table~\ref{tab:relativectr}. The setting of all algorithms with the highest reward is highlighted in bold. Our algorithm \texttt{ICTRUCB(2,10,0.1)} achieves the best performance among all algorithms on Yahoo! Today News, and performance comparisons on different algorithms along different time buckets are shown in Figure~\ref{fig:ydata-performance}. For MovieLens (10M), \texttt{ICTRTS(3,10)} outperforms all others and the corresponding performance comparisons are shown in Figure~\ref{fig:movielen-performance}.


\begin{figure}[htp!]
\centering
  \scalebox{0.22}{
   \includegraphics{fig/ydata_stats-eps-converted-to.pdf}
  }
\vspace{-0.2in}
\caption{The CTR of Yahoo! Today News data is given along each time bucket. All algorithms shown here are configured with their best parameter settings.}
\label{fig:ydata-performance}
\end{figure}

\begin{figure}[htp!]
 \centering
  \scalebox{0.22}{
   \includegraphics{fig/movielen_stats-eps-converted-to.pdf}
  }
\vspace{-0.2in}
\caption{The Rating of MovieLens (10M) data is given along each time bucket. All algorithms shown here are configured with their best parameter settings.}
\label{fig:movielen-performance}
\end{figure}

\begin{table*}[!htb]
        %\small
        \centering
        \caption{Results of Relative CTR (Rating) on two real world datasets}
        \vspace{-0.05in}
        \scalebox{0.9}{
        \begin{tabular}{llllllllll}
        \toprule
        \textbf{Algorithm} & \multicolumn{4}{c}{\textbf{Yahoo! Today News}}  &\quad\quad& \multicolumn{4}{c}{\textbf{MovieLens (10M)}}\\
        \cmidrule(r){2-5} \cmidrule(r){7-10}
           & mean  &  std  & min & max  && mean  &  std  & min & max \\
        \midrule
        \texttt{$\epsilon$-greedy(0.01)} & 0.06916 & 0.00312 & 0.06476 & 0.07166  && 0.70205 & 0.06340 & 0.60752 & 0.78934 \\
        \texttt{$\epsilon$-greedy(0.1)} & \textbf{0.07566} & 0.00079 & 0.07509 & 0.07678   && \textbf{0.82038} & 0.01437 & 0.79435 & 0.83551 \\
        \texttt{$\epsilon$-greedy(0.3)} & 0.07006 & 0.00261 & 0.06776 & 0.07372   && 0.80447 & 0.01516 & 0.77982 & 0.82458 \\
        \texttt{$\epsilon$-greedy(1.0)} & 0.03913 & 0.00051 & 0.03842 & 0.03961   && 0.60337 & 0.00380 & 0.59854 & 0.60823 \\
        \midrule
        \texttt{UCB(0.01)} & 0.05240 & 0.00942 & 0.04146 & 0.06975  && 0.62133 & 0.10001 & 0.45296 & 0.73369 \\
        \texttt{UCB(0.1)} & \textbf{0.08515} & 0.00021 & 0.08478 & 0.08544   && \textbf{0.73537} & 0.07110 & 0.66198 & 0.85632 \\
        \texttt{UCB(0.5)} & 0.05815 & 0.00059 & 0.05710 & 0.05893   && 0.71478 & 0.00294 & 0.63623 & 0.64298 \\
        \texttt{UCB(1.0)} & 0.04895 & 0.00036 & 0.04831 & 0.04932   && 0.63909 & 0.00278 & 0.60324 & 0.61296 \\
        \midrule
        \texttt{TS(0.01,0.01)} & 0.07853 & 0.00058 & 0.07759 & 0.07921   && \textbf{0.83585} & 0.00397 & 0.82927 & 0.84177\\
        \texttt{TS(0.1,0.1)} & \textbf{0.07941} & 0.00040 & 0.07869 & 0.07988   && 0.83267 & 0.00625 & 0.82242 & 0.84001\\
        \texttt{TS(0.5,0.5)}  & 0.07914 & 0.00106 & 0.07747 & 0.08041   && 0.82988 & 0.00833 & 0.81887 & 0.84114\\
        \texttt{TS(1.0,1.0)} & 0.07937 & 0.00079 & 0.07788 & 0.08044   && 0.83493 & 0.00798 & 0.82383 & 0.84477\\
        \midrule
        \texttt{PTS(2,2)} & \textbf{0.06069} & 0.00575 & 0.05075 & 0.06470   && \textbf{0.70484} & 0.03062 & 0.64792 & 0.74610 \\
        \texttt{PTS(2,10)} & 0.05699 & 0.00410 & 0.05130 & 0.06208   && 0.65046 & 0.01124 & 0.63586 & 0.66977 \\
        \texttt{PTS(5,10)} & 0.05778 & 0.00275 & 0.05589 & 0.06251   && 0.63777 & 0.00811 & 0.62971 & 0.65181 \\
        \texttt{PTS(5,20)} & 0.05726 & 0.00438 & 0.05096 & 0.06321   && 0.62289 & 0.00714 & 0.61250 & 0.63567 \\
        \texttt{PTS(10,20)} & 0.05490 & 0.00271 & 0.05179 & 0.05839   && 0.61819 & 0.01044 & 0.60662 & 0.63818 \\
        \midrule
        %\midrule
        \texttt{ICTRTS(2,5)} & 0.06888 & 0.00483 & 0.06369 & 0.07671   && 0.70386 & 0.15772 & 0.48652 & 0.85596 \\
        \texttt{ICTRTS(2,10)} & 0.06712 & 0.01873 & 0.03731 & 0.08487   && 0.56643 & 0.10242 & 0.42974 & 0.67630 \\
        \texttt{ICTRTS(3,10)} & 0.06953 & 0.00783 & 0.05857 & 0.07804   && \textbf{0.88512} & 0.00052 & 0.88438 & 0.88553 \\
        \texttt{ICTRTS(5,10)} & \textbf{0.08321} & 0.08236 & 0.08492 & 0.06292   && 0.55748 & 0.14168 & 0.38715 & 0.73404 \\
        \texttt{ICTRTS(7,10)} & 0.05066 & 0.00885 & 0.04229 & 0.06423   && 0.517826 & 0.07120 & 0.42297 & 0.59454 \\
        \texttt{ICTRTS(7,20)} & 0.04925 & 0.00223 & 0.04672 & 0.05285   && 0.61414 & 0.12186 & 0.44685 & 0.73365 \\
        \midrule
        \texttt{ICTRUCB(2,10,0.01)} & 0.06673 & 0.01233 & 0.04588 & 0.08112   && 0.44650 & 0.06689 & 0.38678 & 0.53991 \\
        \texttt{ICTRUCB(2,10,1.0)} & \textbf{0.08597} & 0.00056 & 0.08521 & 0.08675   && \textbf{0.86411} & 0.01528 & 0.85059 & 0.88547 \\
        \texttt{ICTRUCB(3,10,0.05)} & 0.07250 & 0.00426 & 0.06799 & 0.07694   && 0.54757 & 0.13265 & 0.43665 & 0.73407 \\
        \texttt{ICTRUCB(3,10,1.0)} & 0.08196 & 0.00296 & 0.07766 & 0.08530   && 0.57805 & 0.08716 & 0.46453 & 0.67641 \\
        \texttt{ICTRUCB(5,10,0.01)} & 0.07009 & 0.00722 & 0.06411 & 0.08244   && 0.62282 & 0.02572 & 0.59322 & 0.65594 \\
        \texttt{ICTRUCB(5,10,1.0)} & 0.08329 & 0.00140 & 0.08098 & 0.08481   && 0.80038 & 0.24095 & 0.9625 & 0.88554 \\
        \bottomrule
        \end{tabular}
        }
        \label{tab:relativectr}
\end{table*}

\subsubsection{A Case Study: Movie Topic Distribution Analysis on MovieLens (10M)}
We conduct an experiment to demonstrate that our model can effectively capture the dependency between items, i.e., finding the latent topics among movies and clustering similar movies together. In this experiment, top-N $(N=8)$ popular movies are selected and topic number $(K=2)$ is set as config to our model. After millions of training iterations, the learned latent movie feature vectors will represent each movie's topic distribution over the two latent topics, in which the $i$-th dimension of the feature vector encodes the probability that the movie belongs to the $i$-th movie topic cluster.
%Table~\ref{tab:moviecluster} shows us the information of two movie topic clusters with their movie ids, names and movie types. The two sets separately selects 4 movies with the highest value in the first and the second dimension of their feature vectors. From the ground truth information MovieType, each set clearly represents one type of movies which proves efficacy of our model.
We separately choose four movies with the highest value of the first element and the second element of these latent feature vectors, and list their IDs, names, and movie types in Table~\ref{tab:moviecluster}, which clearly proves our assumption that the model is able to capture the dependency between items and cluster similar movies together.
\begin{table*}[!htb]
        \vspace{-0.1in}
        \centering
        \caption{Movie Topic Distribution of MovieLen (10M)}
        \scalebox{0.9}{
        \begin{tabular}{ccccccc}
        \toprule
        \multicolumn{3}{c}{\textbf{Topic Cluster I}}  &\quad\quad  & \multicolumn{3}{c}{\textbf{Topic Cluster II}} \\
        \cmidrule(r){1-3} \cmidrule(r){5-7}
         MovieId  &  MovieName  & MovieType && MovieId  &  MovieName  & MovieType  \\
        \midrule
         32 & 12 Monkeys & Sci-Fi,Thriller    && 344 & Pet Detective & Comedy \\
         \midrule
         50 & Usual Suspects & Crime,Mystery,Thriller    && 588 & Aladdin & Children,Animation,Comedy \\
         \midrule
         590 & Dances with wolves & Adventure,Drama,Western    && 595 & Beauty and the Beast & Animation,Children,Musical\\
         \midrule
         592 & Batman & Action,Crime,Sci-Fi,Thriller    && 2857 & Yellow Submarine & Adventure,Animation,Comedy,Musical \\
        \bottomrule
        \end{tabular}
        }
        \label{tab:moviecluster}
\end{table*}
\subsubsection{Time Cost}
The time cost for \texttt{ICTRTS} and \texttt{ICTRUCB} on both two data sets is displayed in Figure~\ref{fig:timecost}. It shows that the time costs are increased linearly with the number of particles and dimensions of latent feature vector. MovieLens (10M) costs  much more time than Yahoo! Today New due to a larger amount of items and users. In general, \texttt{ICTRUCB} is faster than \texttt{ICTRTS} since \texttt{ICTRTS} highly depends on the sampling process.
\begin{figure}[htp!]
\centering
\begin{subfigure}{0.23\textwidth}
  \scalebox{0.11}{
   \includegraphics{fig/time-cost-particle-eps-converted-to.pdf}
  }
\label{fig:timecostparticle}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
  \scalebox{0.11}{
   \includegraphics{fig/time-cost-dimension-eps-converted-to.pdf}
  }
\label{fig:timecostdimension}
\end{subfigure}
\vspace{-0.2in}
\caption{Time cost are given with respect to different number of particles and latent feature vector dimensions for both two datasets.}
\label{fig:timecost}
\vspace{-0.2in}
\end{figure}



==> arXiv copy/introduction.tex <==
\section{Introduction} \label{sec:introduction}
The overwhelming amount of data necessitates an efficient online interactive recommendation system where the online users constantly interact with the system, and user feedback is instantly collected for improving recommendation performance.
Online interactive recommender systems are challenged to immediately suggest the consumers with appropriate items (e.g., movies, news articles) according to the current context that includes both the consumer and item content information.
The systems try to continuously maximize the consumers' satisfaction over the long run.
To achieve this goal, it becomes a critical task for recommender systems to track the consumer preferences instantly and to recommend interesting items to the users from a large item repository.

However, identifying the appropriate match between the consumer preferences and the target items is quite difficult for recommender systems due to several existing practical challenges.
One challenge is the well-known \textit{cold-start} problem since a significant number of users/items might be completely new to the system, that is, they may have no consumption history at all.
This problem makes recommender systems ineffective unless additional information about both items and users is collected~\cite{zeng2016online}, \cite{chang2015space}.
The second challenge is that most recommender systems typically assume that the entire set of contextual features with respect to both users and items can be accessed for users' preference inference. %, and the users' preference of the items can be inferred from the context information. %which govern the generation of payoff from a user to an item.
Due to a number of reasons -{}- privacy or sampling constraints are among them -{}- it is challenging to obtain all relevant features ahead of time, thus rendering many factors unobservable to the recommendation algorithms.


In the first challenge, an \textit{exploration} or \textit{exploitation} dilemma is identified in the aforementioned setting. A tradeoff between two competing goals needs to be considered in recommender systems: maximizing user satisfaction using their consumption history, while gathering new information for improving the goodness of match between user preference and items~\cite{li2010contextual}.
 %at expense of users' satisfaction in short term~\cite{li2010contextual}.
 %the long-run consumers' satisfaction maximization and the dynamic context exploration for good match between consumer preferences and items~\cite{li2010contextual}.
 This dilemma is typically formulated as a multi-armed bandit problem where each arm corresponds to one item.
 The recommendation algorithm determines the strategies for selecting an arm to pull according to the contextual information at each trial.
 Pulling an arm indicates that the corresponding item is recommended. When an item matches the user preference (e.g., a recommended news article or movie is consumed), a reward is obtained; otherwise, no reward is provided. The reward information is fed back to the algorithm to optimize the strategies.
 The optimal strategy is to pull the arm with the maximum expected reward with respect to the historical interaction on each trial, and then to maximize the total accumulated reward for the whole series of trials.

% Most contextual bandit algorithms simply assume the learner would have access to the entire set of features, which govern the generation of payoffs from a user to an item. However, in practice it is challenging to exhaust all relevant features ahead of time, and oftentimes due to privacy or sampling constraints many factors are unobservable to the algorithm. Failing to model such hidden factors leads a system to make constantly suboptimal predictions. In this paper, we propose to learn the hidden features for contextual bandit algorithms. Hidden features are explicitly introduced in our reward generation assumption, in addition to the observable contextual features.

\begin{comment}
The growth of the Internet has made it much more difficult to effectively extract interesting or relevant information from all available online information. The overwhelming amount of data necessitates mechanisms for efficient information filtering. Recommender system is one of the mechanisms to deal with this problem and help users discover interesting or relevant information;
%With the continuous growth of online services, it becomes an increasingly important research area on recommender systems which help users discover interesting or relevant information out of a myriad of data;
users can either browse, search or simply receive recommendations to meet their needs. Netflix reported 2/3 rented movies originated from recommended items in 2006~\cite{lamere2008project}, which further motivated Netflix to offer \$1 million prize for the first group to improve their recommendations by 10\%. Meanwhile, Google News traffic has grown by 38\% after adopting its personalized recommender system~\cite{das2007google}.
%Though the adoption of traditional recommendation techniques provide a intelligent way to discover relevant items and achieves a great success, they still face some challenges unresolved.

%the study on recommender systems has become an increasingly important area of research.
%Many online service platforms (e.g. Netflix, Amazon, Yahoo!)~\cite{resnick1997recommender} provide online personalized recommendations to help customers deal with the information overload issue, thus improve customers' experience and increase sales.

%Traditionally, the recommender systems describe a variety of techniques including collaborative filtering, content-based recommendations and hybrid approaches~\cite{adomavicius2005toward}.
\end{comment}
Collaborative filtering (CF), an early recommendation technique, is widely applied in recommender systems to address the second challenge, mentioned above~\cite{schafer2007collaborative},\cite{bennett2007netflix},\cite{koren2009matrix}.
%To address the second challenge, collaborative filtering (CF), one of those early recommendation techniques, %which can be categorized as memory-based approaches and model-based approaches~\cite{adomavicius2005toward}. CF techniques
CF has gained its popularity due to its advantage over other recommendation techniques, where CF requires no extra information about items or users for recommendation but only requires users' historical ratings on items~\cite{kawale2015efficient,herlocker1999algorithmic}. %CF has been extensively used in diverse applications like online e-commerce~\cite{schafer2007collaborative},
Further, considering both aforementioned challenges simultaneously aggravates the difficulties when recommending items.

Recently, an online interactive collaborative filtering system has been suggested~\cite{zhao2013interactive, kawale2015efficient} adopting both techniques, multi-armed bandit and collaborative filtering.
Typically, the collaborative filtering task is formulated as a matrix factorization problem. Matrix factorization derives latent features for both users and items from the historical interaction records.
It assumes that a user's preference (i.e., rating) on a given item can be predicted by considering items' and users' latent feature vectors.
Based on this assumption, multi-armed bandit policies make use of the predicted reward (i.e., user's preference) for arm (i.e., item) selection.
The feedback occurring between the given user and arm is used to update the user's and arm's latent vectors, without impacting the inference of other arms' latent vectors by supposing arms are independent from each other.

However, the assumption about the independency among arms rarely holds in real-world applications. For example, in the movie recommendation scenario, the movies correspond to the arms. The dependent arms (i.e., movies) typically share similar latent topics (e.g., science fiction movies, action movies, etc.), and are likely to receive similar rewards (i.e., ratings or feedbacks) from users. Intuitively, the dependencies among arms can be utilized for reward prediction improvement and further facilitated the maximization of users' satisfaction in the long run.

In this paper, we introduce an interactive collaborative topic regression model that utilizes multi-armed bandit algorithms with dependent arms for the item recommendations to the target user. A sequential online inference method is proposed to learn the latent parameters and infer the latent states. We adopt a generative process based on topic model to explicitly formulate the arm dependencies as the clusters on arms, where dependent arms are assumed to be generated from the same cluster.
Every time an arm is pulled, the feedback is not only used for inferring the involved user and item latent vectors, but it is also employed to update the latent parameters with respect to the arm's cluster. The latent cluster parameters further help with reward prediction for other arms in the same cluster. The fully adaptive online inference strategy of particle learning~\cite{carvalho2010particle} allows our model to effectively  capture the arm dependencies. In addition, the learnt parameters can be naturally integrated into existing multi-arm selection strategies, such as \textit{UCB} and \textit{Thompson sampling}.
We conduct empirical studies on two real-world applications, recommendations of movie and news.
The experimental results demonstrate the effectiveness of our proposed approach.

\begin{comment}
In summary, we make the following contributions:
\begin{itemize}[leftmargin=*]
  \item We explicitly model the arm dependency
  \item We propose an interactive collaborative topic regression (ICTR) model that the first models the dependency among arms in a multi-armed bandit setting thus naturally solve the cold-start problem.
  \item We adopt a sequential online learning technique, particle learning~\cite{carvalho2010particle}, to inference parameters and states for ICTR model which enable sequential recommendations of items to the target user in an online setting.
  \item We conduct extensive experiments for our proposed algorithms on two real world datasets. Experimental results demonstrate not only the effectiveness and efficiency of our approach over the current state-of-arts but also the capability of automatically clustering the arms.
\end{itemize}
\end{comment}


%the inference for one movie are supposed to facilitate the inferences of its dependent  with similar topics are supposed to benefit from one another.
%Therefore, the consuming record about a single item of a specific topic can be utilized to update the latent vector of the item as well as the global distribution of items for the particular topic. The updated distribution further helps to improve the preference prediction about other items within the same topic. Enlightened by the topic model, this paper comes up with a generative model to explicitly capture the dependency among arms.



\begin{comment}

First memory-based CF was proposed by Amazon in the late 1990s and promoted into its many online e-commerce systems~\cite{schafer2007collaborative}.
%Nowadays, collaborative filtering is still considered as an effective and widely used recommendation algorithm.
%Without requiring extra information about either items or users for recommendation, CF analyses historical interaction alone based on ratings or behavior of other users.
Witnessing the great success of collaborative filtering techniques, Netflix published a data set ,containing $100,480,507$ ratings that $480,189$ users gave to $17,770$ movies, for the Netflix Prize, an open competition for the best CF algorithms to predict user ratings for films in 2007~\cite{bennett2007netflix}. The data set now is widely used for evaluating recommender system, particularly CF-based recommender system. Matrix factorization (MF) collaborative filtering has emerged as a powerful framework to perform recommendation~\cite{koren2009matrix} in the Netflix Prize competition.
%, which has been widely used as a large-scale data set for evaluating recommender system.
In MF setting, both users and items are mapped into a low-dimension latent factor space by decomposing a partially-observed rating matrix $\mathbf{R} \in \mathcal{R}^{M \times N}$ into a product of two small matrices, $\mathbf{P} \in \mathcal{R}^{M \times K}$ and $\mathbf{Q} \in \mathcal{R}^{N \times K}$, where $\mathbf{R} = \mathbf{PQ^{T}}$. Due to their effectiveness in various situations, even when the rating matrix $\mathbf{R}$ is quite sparse, a variety of MF-based CF methods have been proposed and studied in the literature~\cite{salakhutdinov2007probabilistic,salakhutdinov2008bayesian,billsus1998learning}. However, they still bear the inability to draw any inferences for users or items which have not yet gathered sufficient information, also known as a cold-start problem. Studies~\cite{zhao2013interactive, kawale2015efficient} naturally leverage multi-armed bandit algorithm to solve the cold-start problem. The multi-armed bandit problem models that the agent/user has to decide which arm/item to pull/recommend, and simultaneously attempts to acquire new knowledge (called \textit{exploration}) and optimize his or her decisions based on existing knowledge (called \textit{exploitation}).

Despite their promising performance, Most traditional recommender systems still suffer from two essential challenges; 1) it is difficult to sequentially recommend items to the target individual in an online setting while rapidly adapting to the user's feedback for better prediction; 2) To the best of our knowledge, the existing prior work on recommender systems with multi-armed bandit setting all assumes that the success probabilities of pulling the arms are independent, which is rarely holding in practice~\cite{pandey2007multi}.

%To address these two challenges, online matrix-factorization recommendation~\cite{zhao2013interactive, kawale2015efficient} has been proposed by combining matrix completion with multi-armed bandit algorithms.
%This mechanism was first introduced in previous work~\cite{zhao2013interactive}, where a framework called Interactive Collaborative Filtering (ICF) is presented to study CF in an interactive setting by integrating probabilistic matrix factorization model and leveraging bandit algorithms such as Thompson sampling (TS)~\cite{chapelle2011empirical} and Upper Confidence Bound (UCB)~\cite{auer2002using} to capture the distribution of user and item feature vector. The common dilemma between \textit{Exploitation} and \textit{Exploration} in recommender systems has been well studied in bandit algorithms for decades, which solve the cold-start problem naturally. However, ICF only provides an appropriate solution to the problem of cold start on the user side and online updates the distribution of user latent feature vector whenever new ratings are collected by the system.
%In~\cite{kawale2015efficient}, authors propose a novel algorithm called Particle Thompson sampling for online MF recommendation by combining of particle filtering and Thompson sampling for online Bayesian parameter estimation in the non-conjugate case. It is also the first work to fully solve these two challenges mentioned before. Although these studies have shown a substantial improvement compared with the tradition MF recommendation, the combined bandit algorithms under the strong assumption that the success probabilities of the arms are independent, which is rarely holding in practice~\cite{pandey2007multi}.
\end{comment}
%In this paper, to exploit dependency among arms in a multi-armed bandit setting, we propose an MF-based recommender system which integrates topic modeling~\cite{blei2003latent} to soft cluster the arms and thus promote each feedback within clusters. In summary, we make the following contributions:


%It is a combination of probabilistic matrix factorization (PMF)~\cite{salakhutdinov2007probabilistic} and latent dirichlet allocation (LDA)~\cite{blei2003latent} base on particle learning and develop an effective online inference algorithm when the posterior does not have a closed form. The fully adaptive re-sample inference strategy of particle learning allows our model to maintain a much better approximation of joint distribution of states and conditional sufficient statistics for fixed parameters. In addition, the learnt parameters can be naturally integrated into bandit settings such as Thompson sampling and UCB to select the arm (item). We conduct empirical experiments on two real-world applications including online personalized advertising~\cite{anagnostopoulos2007just} and news recommendation~\cite{li2010contextual}. The results of experiments demonstrate the effectiveness of our proposed algorithm over the current state-of-arts.

The rest of this paper is organized as follows.
In Section~\ref{sec:relatedwork}, we provide a brief summary of prior work relevant to collaborative filtering, collaborative topic model, multi-armed bandit and the online inference with particle learning.
We formulate the problem in Section~\ref{sec:formulation}.
The solution to the problem is presented in Section \ref{sec:solution}.
Extensive empirical evaluation results are reported in Section \ref{sec:experiment}. Finally, Section \ref{sec:conclusion} concludes the paper.




==> arXiv copy/problem-formulation.tex <==
\section{Problem Formulation}
\label{sec:formulation}

In this section, we provide a mathematical formulation of the interactive collaborative filtering problem as a multi-armed bandit problem.
Then we come up with a new generative model describing explicitly the dependency among arms (i.e. items).
 
A glossary of notations mentioned in this paper is summarized in Table~\ref{tab:notations}.

\begin{table}[!h]
\vspace{-0.15in}
	\centering
	\caption{Important Notations}
    \scalebox{0.9}{
	\begin{tabular}{lp{7.5cm}}
		\toprule
		\textbf{Notation} & \textbf{Description}\\
		\midrule
		$M, N$       & number of rows (users) and columns (items).  \\
		$\mathbf{R} \in \mathcal{R}^{M \times N}$   & the rating matrix. \\
        $\mathbb{S}(t)$ & the sequence of $(n(t-1), r_{m,n(t-1)})$ observed until time $t$.\\
        $n(t)$   & the recommended item index in the $t$-th iteration. \\
        $r_{m,t}$  & the reward of the $m$-th user by pulling the given item in the $t$-th iteration. \\
		$y_{m,t}$  & the predicted rating for the $m$-th user over given item in the $t$-th iteration. \\
        $\pi$ & the policy to recommend items sequentially. \\
        $R_\pi$ & the cumulative rating (reward) of the policy $\pi$. \\
        $K$     & the number of topics and the number of dimensions for latent vectors. \\
		%\midrule
        $\mathcal{P}_{k}$  & the set of particles for the item $k$ and $\mathcal{P}^{(i)}_{k}$.\\
        $\mathbf{p}_m \in \mathcal{R}^K$ & the latent feature vector for the $m$-th user. \\
        $\mathbf{q}_n \in \mathcal{R}^K$ & the latent feature vector for the $n$-th item. \\
        $\mathbf{\Phi}_k \in \mathcal{R}^{N}$ & the item distribution of the $k$-th topic. \\
        $z_{m,t}$ & the latent topic of the $m$-th user in the $t$-th iteration. \\
        $x_{m,t}$ & the selected item of the $m$-th user in the $t$-th iteration.\\
        %\midrule
        $\lambda$ & Dirichlet priors over topics for topic model. \\
        $\eta$ & Dirichlet priors over items for topic model. \\
        $\sigma^2_n$ & the variance of rating prediction. \\
        $\alpha$, $\beta$ & the hyper parameters determine the distribution of $\sigma^2_n$. \\
        $\mathbf{\mu}_\mathbf{q}$, $\mathbf{\Sigma}_\mathbf{q}$ & the hyper parameters determine the gaussian distribution of $\mathbf{q}_n$. \\
		$\xi$ & the observation noise of the rating \\
        \bottomrule
	\end{tabular}
    }
	\label{tab:notations}
	\vspace{-0.15in}
\end{table}

\subsection{Basic Concepts and Terminologies}
\label{subsec:base}
Assume that there are $M$ users and $N$ items in the system. The preferences of the users for the items are recorded by a partially observable matrix $\mathbf{R}=\{r_{m,n}\}\in \mathcal{R}^{M\times N}$, where the rating score $r_{m,n}$ indicates how the user $m$ would like the item $n$. The basic collaborative filtering task is to predict the unknown rating score in light of the observed rating scores in $\mathbf{R}$. However, it is very challenging to fulfill the task in practice due to the high dimensionality and sparsity of the rating matrix. Matrix factorization addresses this challenge by mapping each user $m$ and item $n$ to the latent feature vectors $\mathbf{p}_m \in \mathcal{R}^{K}$ and $\mathbf{q}_n \in \mathcal{R}^{K}$ in a shared low $K$-dimension space (typically, $K \ll M, N$). It assumes that the rating $r_{m,n}$ can be predicted by
\begin{equation}
  \hat{r}_{m,n} = \mathbf{p}_m^\intercal\mathbf{q}_n.
  \label{eq:pq}
\end{equation}
Therefore, the latent features $\{\mathbf{p}_m\}$ and $\{\mathbf{q}_n\}$ can be learned by minimizing the prediction error for all observed ratings in $\mathbf{R}$, while each unobserved rating value can be estimated using Equation~(\ref{eq:pq}) with its corresponding latent features learned by matrix factorization.
In practice, since the feedback (i.e., rating scores) from users is received over time, the recommender system is required to address the collaborative filtering problem in an interactive mode.
The recommender system is referred to as an interactive recommender system.



In an interactive recommender system, a user $m$ constantly arrives to interact with system over time. At each time $t \in [1,T]$, the system, according to the observed rating history, recommends an item $n(t)$ to the corresponding user $m$. After consuming the item $n(t)$, the feedback (i.e., rating) $r_{m,n(t)}$ from the user $m$ is collected by the system and further utilized to update the recommendation model for the next item delivery. The interactive recommendation process involves a series of decisions over a finite but possibly unknown time horizon $T$. Accordingly, we formulate the interactive recommendation process as a multi-armed bandit problem, where each item corresponds to an arm. Pulling an arm indicates that its corresponding item is being recommended, and the rating score is considered as the reward received after pulling the corresponding arm.

Let $\mathbb{S}(t)$ be the available information at time $t$ collected by the system for the target user $m$,
\begin{equation}
 \begin{split}
 \mathbb{S}(t) = \{(n(1), r_{m,n(1)}),\dots,(n(t-1), r_{m, n(t-1)})\}.
 \end{split}
 \end{equation}
A policy $\pi$ is defined as a function and used to select an arm based on the current cumulative information $\mathbb{S}(t)$,
\begin{equation}
 \begin{split}
 n(t) = \pi(\mathbb{S}(t)).
 \end{split}
 \end{equation}
The total reward received by the policy $\pi$ after $T$ iterations is
\begin{equation}
  R_\pi = \sum_{t=1}^{T}{r_{m,\pi(\mathbb{S}(t))}}.
  \label{eq:totalReward}
\end{equation}
The optimal policy $\pi^*$ is defined as the one with maximum accumulated expected reward after $T$ iterations,
\begin{equation}
 \begin{split}
 \pi^* = \arg\max_{\pi}{\mathbb{E}(R_\pi)} = \arg\max_{\pi}\sum_{t=1}^{T}\mathbb{E}(r_{m,\pi(\mathbb{S}(t))}|t).
 \end{split}
 \label{eq:optPolicy}
 \end{equation}
 Therefore, our goal is to identify a good policy for maximizing the total reward.
 Herein we use reward instead of regret to express the objective function, since  maximization of the cumulative rewards is equivalent to minimization of regret during the $T$ iterations~\cite{zhao2013interactive}.

Before selecting one arm at time $t$, a policy $\pi$ typically learns a model to predict the reward for every arm according to the historical accumulated information $\mathbb{S}(t)$.
The reward prediction helps the policy $\pi$ make decisions to increase the total reward.

%The cumulative object function falls into the goal of multi-armed bandit problem, which also maximize the total rewards by pulling the optimal arms during T time stamps.

In the latent factor model~\cite{salakhutdinov2007probabilistic,salakhutdinov2008bayesian}, the rating is estimated by a product of user and item feature vectors $\mathbf{p}_m$ and $\mathbf{q}_n$ in Equation ~(\ref{eq:pq}). %which is widely used in CF algorithms.
From the probabilistic perspective, probabilistic matrix factorization introduces an observation noise $\xi$, a zero-mean Gaussian noise with variance $\sigma^2$~(i.e., $\xi \sim \mathcal{N}(0, \sigma^2)$), to the rating prediction function given in Equation~(\ref{eq:pq}). The derived rating prediction is as follows:
\begin{equation}
 \begin{split}
 r_{m,n} = \mathbf{p}_m^{\intercal}\mathbf{q}_n + \xi.
 \end{split}
 \label{eq:rewardPrediction}
 \end{equation}
In this setting, our objective function in Equation~(\ref{eq:optPolicy}) is re-formulated as:
\begin{equation}
  \begin{split}
 \pi^* = \arg\max_{\pi}\sum_{t=1}^{T}\mathbb{E}_{\mathbf{p}_m,\mathbf{q}_{\pi(\mathbb{S}(t))}}(\mathbf{p}_m^\intercal\mathbf{q}_{\pi(\mathbb{S}(t))}|t).
 \end{split}
 \label{eq:pmfOptPolicy}
\end{equation}
Consequently, the goal of the interactive recommender system is reduced to optimization of the objective function in Equation~(\ref{eq:pmfOptPolicy}).



\textbf{Thompson Sampling,} one of earliest heuristics for the bandit problem~\cite{chapelle2011empirical}, belongs to the probability matching family.
Its main idea is to randomly allocate the pulling chance according to the probability that an arm gives the largest expected reward at a particular time $t$.
Based on the objective function in Equation~(\ref{eq:pmfOptPolicy}), the probability of pulling arm $n$ can be expressed as follows:
\begin{equation}
  \begin{split}
    p(n(t) = n) = \int & {\mathbb{I}[\mathbb{E}(r_{m,n}|\mathbf{p}_m,\mathbf{q}_n)]}) = \max_{i}{\mathbb{E}(r_{m,i}|\mathbf{p}_m,\mathbf{q}_i)}] \\ & p(\mathbf{p}_m,\mathbf{q}_n|t)d\mathbf{p}_md\mathbf{q}_n.
  \end{split}
\end{equation}
At each time $t$, the Thompson sampling algorithm samples both the user and item feature vectors together from their corresponding distributions, and then selects the item that leads to the largest reward expectation.
Therefore, using the Thompson sampling strategy, the item selection function is defined as:
\begin{equation}
  n(t) = \arg\max_{n}{(\mathbf{\tilde{p}}_m^\intercal\mathbf{\tilde{q}}_n|t)},
  \label{eq:funSelection}
\end{equation}
where $\mathbf{\tilde{p}}_m$ and $\mathbf{\tilde{q}}_n$ denote the sampled feature vectors for user $m$ and item $n$, respectively.

To accomplish the Thompson sampling, it is critical to model the random variable $\mathbf{p}_m$ and $\mathbf{q}_n$ using distributions, where the latent feature vectors can be easily sampled and the feedback at every time can be reasonably integrated.
Most of the previous studies suppose a Gaussian prior for both user and item feature vectors, with an assumption that the items are independent from each other~\cite{zhao2013interactive,kawale2015efficient}.
However, this assumption rarely holds in real applications.
In the following section, we explicitly formulate the dependent arms with a generative model.
%In order to sample the latent feature vectors for both user $m$ and item $n$, it's critical to model the random variable $\mathbf{p}_m$ and $\mathbf{q}_n$ with proper distributions, which can be easily updated once new feedback is provided.
%Despite their effectiveness~\cite{zhao2013interactive,kawale2015efficient}, matrix-factorization bandit works under the independent-arm assumption in these systems. In the next section~\ref{subsec:dependence-arm}, both multi-armed bandit with dependent arms and dependence exploitation by topic model will be discussed in our proposed model.
\subsection{Modeling the Arm Dependency} \label{subsec:dependence-arm}

In light of the fact that similar items (i.e., arms) are likely to receive similar feedback (i.e., rewards)% from a particular user
, we assume that a dependency existing among similar items.
The dependencies among items can be further leveraged to improve the users' preferences inference on a particular item even if the item has little historical interaction data in the recommender system.
The challenge here lies in how to sequentially infer the arms' dependencies as well as users' preferences simultaneously, providing the feedback over time.

%Enlightened by the work in ~\cite{pandey2007multi},
In our work, the dependencies among arms are expressed in the form of the clusters of arms, where the dependent arms fall into the same cluster.
In order to explore the dependencies in the multi-armed bandit setting, Latent Dirichlet Allocation (abbr., LDA~\cite{blei2003latent}), a generative statistic model for topic modeling, is adopted to construct the arms' clusters.
We propose the ICTR (\underline{I}nteractive \underline{C}ollaborative \underline{T}opic \underline{R}egression) model to infer the clusters of arms as well as arm selection. %, whose graphic representation is shown in Figure~\ref{fig:model}. %for arm clustering. %by proposing a generative model on clusters of an arms.
%clustering problem.
%in the form of generative model on clusters of arms.

 %Enlightened by the work in ~\cite{pandey2007multi}, we come up with a generative model to cluster all the arms into different groups in an online mode based on the dependency existing between arms.

%arms are expressed as a

%In the previous literature, each item is regarded as an independent arm in the matrix-factorization bandit setting. An optimal recommending policy $\pi$ will choose an item at each time $t \in [1,2, \dots, T]$ by maximizing the cumulative rating (rewards). Recent studies~\cite{zhao2013interactive,kawale2015efficient} present the matrix-factorization bandit algorithms to partially and fully solve the online low-rank matrix completion. However, both of their frameworks leverage independent arms in the bandit setting, where they assume the expected reward of each item is independent and identically distributed. This assumption is rarely holding in practice.
%Therefore, we introduce a novel model to capture the dependence among these items, while solving the problem of fully online matrix completion in the bandit setting. We adopt a typical probabilistic topic model, i.e., Latent Dirichlet Allocation~\cite{blei2003latent}, to construct clusters over items by exploiting the dependence between the items.

The main idea of our model is to treat an item $n$ as a word, and consider a user $m$ as a document.
All the items rated by a user indicate the hidden preferences of the user, analogous to the scenario in topic modeling where the words contained in a document imply its latent topics.
Specifically, let $K$ be the number of latent aspects (i.e., topics or clusters) the users' concern when consuming items.
We assume that $\mathbf{p}_m\in\mathcal{R}^K$ corresponds to the latent vector for user $m$, where the $k$-th component of $\mathbf{p}_m$ suggests the user's preference over the $k$-th aspect of items.
Further, $\mathbf{q}_n\in\mathcal{R}^K$ is supposed to be the latent vector for the item $n$, and the $k$-th component value of $\mathbf{q}_n$ represents the it belongs to the $k$-th cluster.
The rating score $r_{m,n}$, given by user $m$ after consuming item $n$, is assumed to be the inner product of $\mathbf{p}_m$ and $\mathbf{q}_n$. %The rating score prediction problem is reduced to generate latent vectors $\mathbf{p}_m$ and $\mathbf{q}_n$.
By linking to the topic model, a generative process for user ratings is accordingly introduced and presented in Figure~\ref{fig:model}.

\begin{comment}
In our model, an item is treated as a word and the set of the rated item by a user is considered as a document.
In this way, a topic (cluster) is defined as a multinomial distribution over items. Let $\mathbb{\Phi}_k$ denote the $k$-th topic distribution over items shown in Figure~\ref{fig:model} and $\mathbf{\Phi}_{k,n}$ denote the probability of the $n$-th item in the $k$-th topic. At each time $t$, the recommended item $x_{m,t}$ is determined by both topic assignment $z_{m,t}$ and topic distribution $\mathbb{\Phi}_k$ for user $m$, where $x_{m,t} \sim Mult(\mathbf{\Phi}_{z_{m,t}})$. In the following section, we will introduce our proposed model which combines matrix-factorization bandit and probabilistic topic modeling.
\end{comment}
%\subsection{Interactive Collaborative Topic Regression Model} \label{subsec:model}
\begin{comment}
In this section, we introduce our  Interactive Collaborative Topic Regression (ICTR) model by integrating matrix factorization with topic modeling in a bandit setting. Figure~\ref{fig:model} shows the graph model. It is the first approach to combining matrix-factorization bandit and topic modeling to fit a model that can use the latent topic space to explain the observed ratings and the observed items.
\end{comment}
 \begin{figure}[!htb]
    \centering
    \scalebox{0.6}{
        \includegraphics {fig/model-eps-converted-to.pdf}
				%\includegraphics [width=0.8\linewidth, bb=17 3 544 410] {fig/simplified_model.pdf}
    }
    \caption{The graphic model for the ICTR model. Random variable is denoted as a circle. The circle with filled color denotes the observed random variable. Red dot represents a hyper parameter.}
    \label{fig:model}
\end{figure}

\begin{comment}
ICTR model represents a user with topic interests and assumes that the set of the rated items by a user is generated by a topic model over time. For example, we use the latent user feature vector $\mathbf{p}_m \in \mathbb{R}^{K}$ as the topic proportion over the $K$ topics as well as the connection between two models. That's why we call the model interactive collaborative topic regression. The generative process can be described as follows.
\\
  1.  For each topic $k = 1,...,K$.

  (1) Draw $\mathbf{\Phi}_k$ $\sim$ $Dir(\mathbf{\eta})$
  \\
  2.  For each item $n = 1,..,N$.

  (1) Draw the topic-specific item latent vector from

  $\mathbf{q}_n \sim P(\mathbf{q}_n|\mathbf{\mu}_\mathbf{q}, \mathbf{\Sigma}_\mathbf{q}, \sigma^2_n)$, where $p(\sigma^2_n|\alpha, \beta) \sim \mathcal{IG}(\alpha, \beta)$.
  \\
  3. For each user $m = 1,...,M$.

  a. Draw user latent vector $\mathbf{p}_m \sim Dir(\mathbf{\lambda})$

  b. For $t = 1,2,...,T$.

  \setlength\parindent{3em} (1) Draw a topic assignment $z_{m, t} \sim Mult(\mathbf{p}_{m})$

  \setlength\parindent{3em} (2) Draw $x_{m,t} \sim Mult(\mathbf{\Phi}_{z_{m,t}})$

  \setlength\parindent{3em} (3) The predicted rating $y_{m,t} \sim N(y_{m,t} | {\mathbf{p}_{m}^{\intercal}} \mathbf{q}_{x_{m,t}}, \sigma^2_n)$

  \setlength\parindent{3em} where $p(\sigma^2_n|\alpha, \beta) \sim \mathcal{IG}(\alpha, \beta)$.
\\
\noindent \ \ \ \ In our graphical model, the predicted rating $y_{m,t}$ depends on random variable $\mathbf{p}_m$, $\mathbf{q}_n$ and $\sigma^2_n$ formally given as follows:
 \begin{equation}
   p(y_{m,t}|\mathbf{p}_m, \mathbf{q}_{x_{m,t}}, \sigma^2_n) = N(y_{m,t} | {\mathbf{p}_{m}^{\intercal}} \mathbf{q}_{x_{m,t}}, \sigma^2_n)
  \label{eq:pmfrating}
\end{equation}

 \noindent \ \ \ \ A policy $\pi$ selects one item $n(t)$ to pull according to the reward prediction model. After pulling the item $n(t)$ at time $t$, a corresponding reward $r_{m, t}$ is observed, while the rewards of other items are still hidden. A new element $(n(t),r_{m,n(t)})$ is obtained and a new sequence $\mathbb{S}(t+1)$ is formed by combining $\mathbb{S}(t)$.

\noindent \ \ \ \ The key property in ICTR model lies in how the user/item feature vector is generated. Both $\mathbf{p}_m \in \mathbb{R}^K$ and $\mathbf{q}_n \in \mathbb{R}^K$ are random variables following certain distribution $p(\mathbf{p}_m, \mathbf{q}_n|t)$. For Equation~\ref{eq:optPolicy}, a heuristic solution can be obtained by sampling an item according to its probability of being optimal~\cite{chapelle2011empirical}.
\end{comment}

Based on the above description, the user latent vector $\mathbf{p}_m$ is assumed to follow a Dirichlet prior distribution with a predefined hyper parameter $\mathbf{\lambda}$, shown in Equation~\ref{eq:pmPrior}. %At time $t$, the user $m$ arrives to interact with the recommender system. The latent preference of $m$ is assumed to be generated with a Dirichlet prior distribution ruled by the hyper parameter $\lambda$.
\begin{equation}
 \mathbf{p}_m|\mathbf{\lambda} \sim Dir(\mathbf{\lambda}).
 \label{eq:pmPrior}
 \end{equation}
 %where $\lambda$ is the predefined hyper parameter.
As presented in Equation~\ref{eq:rewardPrediction}, we denote $\mathbf{\sigma}^2$ as the variance of the noise for reward prediction, and we assume $\sigma^2_n$ is drawn from the Inverse Gamma (abbr., $\mathcal{IG}$) distribution shown in Equation~\ref{eq:deltaPrior}.
\begin{equation}
 p(\sigma^2_n|\alpha, \beta) = \mathcal{IG}(\alpha, \beta),
 \label{eq:deltaPrior}
\end{equation}
where $\alpha$ and $\beta$ are the predefined hyper parameters for the Inverse Gamma distribution.

Given $\mathbf{\sigma}^2_n$, the item latent vector $\mathbf{q}_n$ is generated by a Gaussian prior distribution as follows:
\begin{equation}
\mathbf{q}_{n}|\mathbf{\mu}_\mathbf{q}, \mathbf{\Sigma}_\mathbf{q}, \sigma^2_n \sim \mathcal{N}(\mathbf{\mu}_\mathbf{q}, \sigma^2_n\mathbf{\Sigma}_\mathbf{q}),
 \label{eq:itemDistribution}
 \end{equation}
where $\mathbf{\mu}_\mathbf{q}$ and $\mathbf{\Sigma}_\mathbf{q}$ are predefined hyper parameters.

Further, let $\mathbf{\Phi}_k\in\mathcal{R}^N$ be the item distribution for the topic $k$.
Similar to $\mathbf{p}_m$, Dirichlet distribution is specified as the prior of $\mathbf{\Phi}_k$ shown in Equation~\ref{eq:phiPrior}
\begin{equation}
  \mathbf{\Phi}_k|\eta \sim Dir(\eta),
  \label{eq:phiPrior}
\end{equation}
where $\eta\in\mathcal{R}^N$ is the hyper parameter.

When user $m$ arrives to interact with the recommender system at time $t$, one of $K$ topics, denoted as $z_{m,t}$, is first selected according to the user's latent preference $\mathbf{p}_m$, indicating that the user $m$ shows interest in the topic $z_{m,t}$ at this moment.
Accordingly, $z_{m,t}$ is supposed to follow a multinomial distribution governed by $\mathbf{p}_m$ as follows,
\begin{equation}
  z_{m,t}|\mathbf{p}_m \sim Mult(\mathbf{p}_m).
  \label{eq:zDistr}
\end{equation}

Without loss of generality, we assume $z_{m,t} = k$, then the item distribution for the topic $k$ (i.e., $\mathbf{\Phi}_k$) is used for generating the item $x_{m,t}$ recommended to the user $m$ at time $t$.
We assume the random variable $x_{m,t}$ follows the multinominal distribution ruled with $\mathbf{\Phi}_k$, i.e.,
\begin{equation}
  x_{m,t}|\mathbf{\Phi}_k \sim Mult(\mathbf{\Phi}_k).
  \label{eq:xDistr}
\end{equation}

Without loss of generality, item $n$ is assumed to be selected by user $m$ at time $t$ (i.e., $x_{m,t}=n$) where the latent vector corresponding to item $n$ is $\mathbf{q}_n$.  Let $y_{m,t}$ be the predicted reward (i.e., rating), given by user $m$ at time $t$. The predicted reward $y_{m,t}$ can be inferred by
\begin{equation}
  y_{m,t} \sim \mathcal{N}(\mathbf{p}_m^\intercal\mathbf{q}_n, \sigma^2_n).
  \label{eq:predictedReward}
\end{equation}
By Equation~\ref{eq:predictedReward}, the rewards of different items are predicted. Based on the predicted rewards, the policy $\pi$ selects an item and recommends it to the user $m$, considering the trade-off between exploitation and exploration. After consuming the recommended item, the recommender system receives the actual reward $r_{m,t}$ from the user. The objective of the model is to maximize the expected accumulative rewards in the long run as described in Equation~\ref{eq:optPolicy}.


\begin{comment}
\noindent \ \ \ \ In the following, we introduce how to model the interactive recommendation and dependence relationship among items. At each time $t \in [1,2,\dots,T]$, our system will recommend an item $n(t)$ according to the current user's preference $\mathbf{p}_m$. We utilize the topic model to learn the user's preference, dependence among items, and recommend the ``best" item to the current user. Let $z_{m,t}$ represent the $t$-th latent topic drawn from the multinomial distribution with hyper parameter $\mathbf{p}_m$ as follows:
\begin{equation}
 \begin{split}
 p(z_{m,t}|\mathbf{p}_m) = Mult(\mathbf{p}_m)
 \end{split}
\end{equation}

\noindent \ \ \ \ Assuming there are K topics (cluster) in our model, $\Phi_k$ denotes the $k$-th topic distribution over items also drawing from a Dirichlet distribution with hyper parameter $\eta$:
\begin{equation}
 \begin{split}
 p(\mathbf{\Phi}_{k}|\eta) = Dir(\eta)
 \end{split}
\end{equation}
Then we can sample an item at the $t$-th iteration from a multinomial distribution below:
\begin{equation}
 \begin{split}
 p(x_{m,t}|z_{m,t}, \mathbf{\Phi}_k) = Mult(\mathbf{\Phi}_{z_{m,t}})
 \label{eq:itemindex}
 \end{split}
\end{equation}
Combining the Equation~\ref{eq:itemDistribution}, we can obtain the item feature vector distribution $\mathbf{q}_n$ as follows:
\begin{equation}
 \begin{split}
 p(\mathbf{q}_n|x_{m,t},\mathbf{\mu}_\mathbf{q}, \mathbf{\Sigma}_\mathbf{q}, \sigma^2_n) = \mathcal{N}(\mathbf{\mu}_{\mathbf{q}_{x_{m,t}}}, \sigma^2_n\mathbf{\Sigma}_{\mathbf{q}_{x_{m,t}}})
 \label{eq:itemdistribution}
 \end{split}
\end{equation}
\end{comment}

In this section, taking the clusters of arms into account, we formally introduce our ICTR model, which integrates matrix factorization with topic modeling under the multi-armed bandit setting. We develop our solution to infer the ICTR model from a Bayesian perspective and the solution is presented in the following section.






==> arXiv copy/relatedwork-bak.tex <==
\section{Related Work} \label{sec:relatedwork}
In this paper, we come up with an interactive collaborative topic regression model recommending an item to the user in an interactive way by leveraging multi-armed bandit algorithms with dependent arms. Also, a sequential online inference method is proposed to learn the latent unknown parameters and infer the latent states. In this section, we highly review the existing works that related to our approach.

\subsection{Recommendation by Matrix Factorization}
%% cf
The collaborative filtering (CF) methods play a central role to recommenders system. Without need for extra information about either items or users, CF recommends items to a target user based on patterns of ratings. There are two primary categories of CF technologies: The memory-based methods~\cite{sarwar2001item, herlocker1999algorithmic} focus on making the recommendation by modeling the relationships between similar items or users, while the model-based methods~\cite{salakhutdinov2007probabilistic, salakhutdinov2008bayesian, agarwal2009regression, ungar1998clustering} provide an alternative approach by developing a model of user ratings. For instance, latent factor models provides better recommendation by projecting both users and items into the a shared low-dimension latent factor space.
%% mf challenge cold-start problem online setting

Among the latent factor models, the matrix factorization~\cite{koren2009matrix} technologies have gained popularity recently due to Netflix Prize and other recommendation competitions. Probabilistic Matrix Factorization (PMF)~\cite{salakhutdinov2007probabilistic} proposes a probabilistic linear algorithm to model observed ratings with Gaussian observation noise. Bayesian Probabilistic Matrix Factorization (BPMF)~\cite{salakhutdinov2008bayesian} presents a fully Bayesian treatment of the Probabilistic Matrix Factorization (PMF) model. Notwithstanding the MF-based methods have been successfully applied into various recommender systems, one of the key challenges faced by these methods is to how to effectively recommend when a new user/item arrives in the recommender system, also referred as cold-start problem. Interactive Collaborative Filtering (ICF)~\cite{zhao2013interactive} studies collaborative filtering in an interactive setting by integrating PMF framework and leveraging multi-armed bandit algorithms to resolve the cold-start problem only considering the user side. Another challenge is to sequentially recommend items to the target user in an online setting and instantly adapt the up-to-date feedback to refine the recommendation predictions. Many real world applications including online personalized advertising and news recommendation try to continuously maximize the consumers' satisfaction in the long run~\cite{zeng2016online}. Particle Thompson Sampling for MF~\cite{kawale2015efficient} studies Rao-Blackwellized particle based on Thompson sampling framework for online matrix factorization.

\subsection{Matrix Factorization with Probabilistic Topic Models}
Recently, several attempts~\cite{wang2011collaborative,purushotham2012collaborative} have been made by researchers to combine collaborative filtering based on matrix factorization and topic modeling~\cite{blei2003latent}. The central idea behind these methods is to leverage topic modeling to capture items content information in latent topic space and focus on combining the merits of both traditional collaborative filtering and probabilistic topic modeling approaches. Different from the above studies, topic modeling is utilized to soft cluster items as topics based on local matrix factorization~\cite{wangbayesian}.

\subsection{Multi-armed Bandit Algorithms}
The recommender systems are required to balance the tradeoff between \textit{exploration} and \textit{exploitation}: maximizing user satisfaction using the history records, while gathering new information for improving recommendation predictions between user preference and items. This dilemma has been well dealt with by a series of multi-armed bandit algorithms including $\epsilon$-greedy algorithm~\cite{tokic2010adaptive}, upper confidence bound (UCB)~\cite{auer2002using}, EXP3~\cite{auer2002nonstochastic} and Thompson sampling~\cite{chapelle2011empirical}.

%$\epsilon$-greedy algorithm is a simple bandit policy by choosing the best arm (the highest average reward) with probability $1-\epsilon$ and randomly
%playing an arm with probability $\epsilon$. UCB policy leverages upper confidence bounds for \textit{exploration} and \textit{exploitation} dilemma and achieves a regret bound of $O(n\sqrt{T})$~\cite{auer2002using}. Thompson sampling~\cite{chapelle2011empirical} is a more flexible algorithm by randomly allocating the pulling chance according to the probability that an arm provides the highest expected reward. In~\cite{zhao2013interactive}, Thompson sampling is applied to model their interaction by considering the distribution of latent feature vectors of both the user and the item.

% contextual multi-armed bandit
 Online personal advertising~\cite{anagnostopoulos2007just,tang2015personalized,zeng2016online} and news article recommendation~\cite{li2010contextual,tang2015personalized,zeng2016online} have successfully engaged contextual multi-armed bandit algorithms to address the cold-start problem, where the contextual features including the user information (e.g., demographic information and behavior targeting features) and item description (e.g., category and type information), are utilized for arm selection.
% multi-armed bandit with dependent arms

However, most of the prior bandit problems focuses on independent arms. A delicate framework~\cite{pandey2007multi} is developed to study the bandit problems with dependent arms, where the dependencies are in the form of a generative model on clusters of arms.
\subsection{Sequential Online Inference}
Sequential online inference algorithm is well developed to learn the latent unknown parameters and infer the latent states in our model. Sequential monte carlo sampling~\cite{halton1962sequential, doucet2001introduction} and particle learning~\cite{carvalho2010particle} are both popular sequential learning methods.

Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution to address the filtering problem~\cite{doucet2000sequential}. By using these methods, discrete time dynamic models typically both nonlinear and non-Gaussian are allowed inference for full posterior distributions.
Particle learning (PL) provides state filtering, sequential parameter learning and smoothing in a large class of state space models~\cite{carvalho2010particle}. Particle learning is an approach approximating the sequence of filtering and smoothing distributions in light of parameter uncertainty for a wide class of state space models.  The central idea behind PL is the creation of a particle algorithm that directly samples from the particle approximation to the joint posterior distribution of states and conditional sufficient statistics for fixed parameters in a fully-adapted re-sample propagate framework.





==> arXiv copy/relatedwork.tex <==
\section{Related Work} \label{sec:relatedwork}
In this section, we highly review the existing works that related to our approach.

\subsection{Interactive Collaborative Filtering}
%% cf
Collaborative filtering (CF) methods play a key role in recommender systems that recommend items to a target user only based on users' historical ratings of items. There are two primary categories of CF technologies: the memory-based methods~\cite{sarwar2001item, herlocker1999algorithmic} 
%mainly make a recommendation by computing the similarity between items or users, while 
and the model-based methods~\cite{salakhutdinov2007probabilistic, salakhutdinov2008bayesian}.
%develop models using data mining and machine learning techniques to find patterns based on ratings. In addition, it handles the sparsity better than memory-based methods such as matrix factorization ~\cite{koren2009matrix} (MF) technologies, which project both users and items into a shared low dimension latent factor space. Our proposed approaches are related to the model-based methods.

Matrix factorization (MF), one of the model-based methods gained popularity due to the Netflix Prize and other recommendation competitions. A significant variety of MF-based methods are proposed.
Probabilistic Matrix Factorization (PMF)~\cite{salakhutdinov2007probabilistic} models the ratings as products of users' and items' latent features considering Gaussian observation noise.
%PMF can scale linearly with number of observations and perform well on very sparse and imbalanced data.
Bayesian Probabilistic Matrix Factorization (BPMF)~\cite{salakhutdinov2008bayesian} presents a fully Bayesian treatment of the PMF model with priors controlling model complexity automatically. 
%Notwithstanding the fact that MF-based methods have been successfully applied into various recommender systems,
However, one of the key challenges existing in the aforementioned methods is an effective recommendation for a new user/item in recommender systems, also referred to as a cold-start problem~\cite{li2010contextual}. Another challenge is to sequentially recommend items to the target user in an online setting and instantly adapt the up-to-date feedback to refine the recommendation predictions. Multi-armed bandit algorithms~\cite{tokic2010adaptive,auer2002using,auer2002nonstochastic,chapelle2011empirical} are widely applied to address the cold-start problem and balance the tradeoff between \textit{exploration} and \textit{exploitation} in online recomemnder systems~\cite{li2010contextual,tang2015personalized,zeng2016online}.
Interactive Collaborative Filtering (ICF)~\cite{zhao2013interactive} tackles these problems in a partially online setting leveraging PMF framework and bandit algorithms. Rao-Blackwellized particle based on Thompson sampling~\cite{chapelle2011empirical} is proposed for a fully online MF recommendation~\cite{kawale2015efficient}.

However, most of the prior bandit problems focus on independent arms. A delicate framework~\cite{pandey2007multi} is developed to study the bandit problems with dependent arms, where the dependencies are in the form of a generative model on clusters of arms. Recently, several attempts~\cite{wang2011collaborative,purushotham2012collaborative,wangbayesian} have been made by researchers to integrate CF based on MF and topic modeling~\cite{blei2003latent} in an offline setting. The central idea behind these methods is to leverage topic modeling to capture item's content information in latent topic space to soft cluster items, and focus on combining the merits of both traditional CF and probabilistic topic modeling. Different from the above mentioned work, we proposed an ICTR (\underline{I}nteractive \underline{C}ollaborative \underline{T}opic \underline{R}egression) model that adopts a generative process based on topic modeling to explicitly formulate the arm dependencies as the clusters on arms in an online setting. 

\subsection{Sequential Online Inference}
Sequential online inference algorithm is well developed to learn the latent unknown parameters and infer the latent states in our model. Sequential monte carlo sampling~\cite{halton1962sequential, doucet2001introduction} and particle learning~\cite{carvalho2010particle} are both popular sequential learning methods. Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution to address the filtering problem~\cite{doucet2000sequential}. 
%By using these methods, discrete time dynamic models typically both nonlinear and non-Gaussian are allowed inference for full posterior distributions. 
Particle learning (PL) provides state filtering, sequential parameter learning and smoothing in a large class of state space models~\cite{carvalho2010particle,zeng2016onlinebigdata}, which is an approach approximating the sequence of filtering and smoothing distributions in light of parameter uncertainty for a wide class of state space models.  The central idea behind PL is the creation of a particle algorithm that directly samples from the particle approximation to the joint posterior distribution of states and conditional sufficient statistics for fixed parameters in a fully-adapted re-sample propagate framework.





==> arXiv copy/relatedwork1.tex <==
\section{Related Work} \label{sec:relatedwork}
%In this paper, we introduce an interactive collaborative topic regression model that utilizes multi-armed bandit algorithms with dependent arms for the item recommendations to the target user.
%A sequential online inference method is proposed to learn the latent parameters and infer the latent states.
In this section, we review the existing work related to our approach.
\subsection{Collaborative Filtering}
%% cf
Collaborative filtering (CF)~\cite{linden2003amazon} methods play a key role in recommender systems
%. Without need for extra information about either items or users, CF
that recommend items to a target user only based on users' historical ratings of items. There are two primary categories of CF technologies. The memory-based methods~\cite{sarwar2001item, herlocker1999algorithmic} focus on making a recommendation by computing the similarity between items or users, while the model-based methods~\cite{salakhutdinov2007probabilistic, salakhutdinov2008bayesian, agarwal2009regression, ungar1998clustering} develop models using data mining and machine learning techniques to find patterns based on ratings. In addition, it handles the sparsity better than memory-based methods such as matrix factorization ~\cite{koren2009matrix} (MF) technologies, which project both users and items into a shared low dimension latent factor space.
%. For instance, latent factor models provide better recommendation by projecting both users and items into a shared low-dimension late\nt factor space.
%% mf challenge cold-start problem online setting

The matrix factorization technologies gained popularity due to the Netflix Prize and other recommendation competitions.
A significant  variety of MF-based methods are proposed.
Probabilistic Matrix Factorization (PMF)~\cite{salakhutdinov2007probabilistic} models the ratings as products of users' and items' latent features and adds Gaussian observation noise.
PMF can scale linearly with number of observations and perform well on very sparse and imbalanced data.
%A fully Bayesian treatment of PMF (BPMF)~\cite{salakhutdinov2008bayesian} present
Bayesian Probabilistic Matrix Factorization (BPMF)~\cite{salakhutdinov2008bayesian} presents a fully Bayesian treatment of the PMF model with priors controlling model complexity automatically.
%Notwithstanding the fact that MF-based methods have been successfully applied into various recommender systems,
However, one of the key challenges existing in the aforementioned methods is effective recommendation for users or items that have not yet gathered sufficient rating information.
This challenge is usually referred to as a cold-start problem.
Interactive Collaborative Filtering (ICF)~\cite{zhao2013interactive} tackles the cold-start problem in an interactive setting by integrating PMF framework and multi-armed bandit algorithms only considering the user side. Particle Thompson Sampling for MF [15] studies Rao-Blackwellized particle based on Thompson sampling framework for online matrix factorization.
Studies~\cite{zeng2016online, kawale2015efficient} undertake the online personalized advertising and news article recommendation tasks~\cite{anagnostopoulos2007just,tang2015personalized,li2010contextual} in an online setting where the model instantly adopts up-to-date feedback to refine the recommendation predictions.
The incorporation of the up-to-date feedback is implemented by sequential online inference techniques.
Moreover, they used contextual multi-armed bandit algorithms to address the cold-start problem, by selecting arms based on the contextual features of the users' information and items' description.

\subsection{Sequential Online Inference \& Multi-armed Bandit Algorithms}
Sequential online inference techniques are well developed for learning the latent parameters and inferring the latent states.
One such technique is sequential Monte Carlo sampling~\cite{halton1962sequential, doucet2001introduction, carvalho2010particle}.
Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution for addressing the filtering problem~\cite{doucet2000sequential}. By using these methods, discrete time dynamic models, typically both nonlinear and non-Gaussian, are allowed to inference for full posterior distributions.
%
Multi-armed bandit algorithms are designed to deal with the demand of balancing the tradeoff between \textit{exploration} and \textit{exploitation} in a recommender system that requires maximizing user satisfaction using history records, while gathering new information for improving recommendation predictions between user preference and items. Classical multi-armed bandit algorithms include $\epsilon$-greedy algorithm~\cite{tokic2010adaptive}, upper confidence bound (UCB)~\cite{auer2002using}, EXP3~\cite{auer2002nonstochastic} and Thompson sampling~\cite{chapelle2011empirical}.

\begin{comment}
\subsection{Sequential Online Inference}
Sequential online inference algorithm is well developed for learning the latent unknown parameters and inferring the latent states in our model. Sequential monte carlo sampling~\cite{halton1962sequential, doucet2001introduction} and particle learning~\cite{carvalho2010particle} are both popular sequential learning methods.

Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution for addressing the filtering problem~\cite{doucet2000sequential}.
Usage of these methods allows inference of the full posterior distributions for the discrete time dynamic models both nonlinear and non-Gaussian.

Particle learning (PL) provides state filtering, sequential parameter learning and smoothing in a large class of state space models~\cite{carvalho2010particle}.
Particle learning is an approach approximating the sequence of filtering and smoothing distributions with parameter uncertainty for a wide class of state space models.
The central idea behind PL is the creation of a particle algorithm that directly samples from the particle approximation to the joint posterior distribution of states and generates sufficient statistics for fixed parameters in a fully-adapted re-sample propagation framework.
\end{comment}

%Another challenge is to sequentially recommend items to the target user in an online setting and instantly adopt the up-to-date feedback to refine the recommendation predictions. Many real world applications including online personalized advertising and news recommendation continuously maximize the consumers' satisfaction in the long run~\cite{zeng2016online}. Particle Thompson Sampling for MF~\cite{kawale2015efficient} studies Rao-Blackwellized particle based on Thompson sampling framework for online matrix factorization.

%\subsection{Matrix Factorization with Probabilistic Topic Models}
Recently, several attempts~\cite{wang2011collaborative,purushotham2012collaborative,wangbayesian} have been made by researchers to model the dependence between items utilizing topic modeling~\cite{blei2003latent} in MF-based Collaborative filtering.
The core idea behind these methods is to apply topic modeling on items' content information to softly cluster items and share the feedback among clusters.
%focus on combining the merits of both traditional collaborative filtering and probabilistic topic modeling approaches.
%Different from the above studies, topic modeling is utilized to soft cluster items as topics based on local matrix factorization~\cite{wangbayesian}.
Different from the above studies, our method not only needs no items' content information to model the dependence between items, but also recommend items in MF-based collaborative filtering with an online setting.

\begin{comment}
\subsection{Multi-armed Bandit Algorithms}
The recommender systems are required to balance the tradeoff between \textit{exploration} and \textit{exploitation}: maximizing user satisfaction using the history records, while gathering new information for improving recommendation predictions between user preference and items. This dilemma has been well dealt with by a series of multi-armed bandit algorithms including $\epsilon$-greedy algorithm~\cite{tokic2010adaptive}, upper confidence bound (UCB)~\cite{auer2002using}, EXP3~\cite{auer2002nonstochastic} and Thompson sampling~\cite{chapelle2011empirical}.


$\epsilon$-greedy algorithm is a simple bandit policy by choosing the best arm (the highest average reward) with probability $1-\epsilon$ and randomly
playing an arm with probability $\epsilon$. UCB policy leverages upper confidence bounds for \textit{exploration} and \textit{exploitation} dilemma and achieves a regret bound of $O(n\sqrt{T})$~\cite{auer2002using}. Thompson sampling~\cite{chapelle2011empirical} is a more flexible algorithmthat  randomly allocates the pulling chance according to the probability that an arm provides the highest expected reward. In~\cite{zhao2013interactive}, Thompson sampling is applied to modelling their interaction by considering the distribution of latent feature vectors of both the user and the item.

% contextual multi-armed bandit
 Online personal advertising~\cite{anagnostopoulos2007just,tang2015personalized,zeng2016online} and news article recommendation~\cite{li2010contextual,tang2015personalized,zeng2016online} have successfully engaged contextual multi-armed bandit algorithms to address the cold-start problem, where the contextual features include the user information (e.g., demographic information and behavior targeting features) and item description (e.g., category and type information), are utilized for arm selection.
% multi-armed bandit with dependent arms

However, most of the prior bandit problems focuses on independent arms. A delicate framework~\cite{pandey2007multi} is developed to study the bandit problems with dependent arms, where the dependencies are in the form of a generative model on clusters of arms.
\end{comment}






==> arXiv copy/solution.tex <==
\section{Methodology and Solution}\label{sec:solution}
In this section, we present the methodology for online inferences of the interactive collaborative topic regression model.

The posterior distribution inference involves five random variables, i.e., $\mathbf{p}_{m}$,
$z_{m,t}$, $\mathbf{\Phi}_{k}$, $\mathbf{q}_n$, and ${\sigma^2_n}$. According to the graphical model in Figure~\ref{fig:model}, the five random variables belong to two categories: parameter random variable and latent state random variable.
$\mathbf{\Phi}_{k}$, $\mathbf{p}_m$, $\mathbf{q}_n$, and ${\sigma^2_n}$ are parameter random variables since they are assumed to be fixed but unknown, and their values do not change with time.
Instead, $z_{m,t}$ is referred to as a latent state random variable since it is not observable and its value is time dependent.
After pulling the arm $n(t)$, where $n(t) = x_{m,t}$ according to Equation~\ref{eq:xDistr} at time $t$, a reward is observed as $r_{m,t}$.
Thus, $x_{m,t}$ and $r_{m,t}$ are referred to as observed random variables.

Our goal is to infer both latent parameter variables and latent state random variable to sequentially fit the observed data at time $t-1$, and predict the rewards for arm selection with respect to the coming user at time $t$. However, since the inference of our model cannot be conducted by a simple closed-form solution, we adopt the sequential sampling-based inference strategy that is widely used in sequential Monte Carlo sampling~\cite{smith2013sequential}, particle filtering~\cite{djuric2003particle}, and particle learning~\cite{carvalho2010particle} to learn the distribution of both the parameter and the state random variables.
Specifically, a particle learning method that allows both state filtering and sequential parameter learning simultaneously is a perfect solution to our proposed model inference.

% However, since the inference partially depends on the random walk which generates the latent state variable, we use the sequential sampling based inference strategy that are widely used sequential monte carlo sampling~\cite{smith2013sequential}, particle filtering~\cite{djuric2003particle}, and particle learning~\cite{carvalho2010particle} to learn the distribution of both parameter and state random variables.
%Particularly,
\begin{comment}
Since the states $\mathbf{p}_{m,t-1}$ and $z_{m,t-1}$ changes over time,  $\mathbf{p}_{m,k}$ follows $P(\mathbf{p}_{m,t-1}|S^{\mathbf{p}_{m,k}}_{t-1})$ and $z_{m,t-1}$ is a value calculated by two latent states $S^{\Phi_{k,n}}_{t-1}$ and $S^{\mathbf{p}_{m,k}}_{t-1}$ after $t-1$ iterations, where $k = z_{m, t-1}$ and n = $x_{m, t-1}$. A particle is defined as follows.
\end{comment}
In order to develop the solution based on the particle learning, we first define the particle as follows.
\begin{definition}[Particle] A particle for predicting the reward $y_{m,t}$ is a container that maintains the current status information for both user $m$ and item $x_{m,t}$. The status information comprises of random variables such as $\mathbf{p}_{m}$,
${\sigma^2_n}$, $\mathbf{\Phi}_{k}$, $\mathbf{q}_n$, and $z_{m,t}$, as well as the hyper parameters of their corresponding distributions, such as $\mathbf{\lambda}$, $\alpha$, $\beta$, $\mathbf{\eta}$, $\mathbf{\mu}_\mathbf{q}$ and $\mathbf{\Sigma_q}$.
\end{definition}
\begin{comment}
the pair of user $m$ and item $n$ is a container which maintains the current status information of the $n$-th item ($n \in [1,2 \dots, N]$). The status information comprises of random variables such as $\mathbf{p}_{m}$, $z_{m,t}$, $\mathbf{\Phi}_{k}$, $\mathbf{q}_n$, and ${\sigma^2_n}$, and the parameters of their corresponding distributions such as $\mathbf{\lambda}$, $\mathbf{\eta}$, $\mathbf{\mu}_\mathbf{q}$ and $\mathbf{\Sigma}_\mathbf{q}$, $\alpha$ and $\beta$.
\end{comment}
In particle learning, each particle corresponds to a sample for modeling inference status information.
At each time stamp, the particles are re-sampled according to their fitness to the current observable data.
Then, the re-sampled particles are propagated to new particles and obtain the status information for the next time stamp.

In the following subsections, we develop our solution based on particle learning.

\subsection{Re-sample Particles with Weights}
At time $t-1$, a fixed-size set of particles is maintained for the reward prediction for each arm $n(t-1)$ given the user $m$. We denote the particle set at time $t-1$ as $\mathcal{P}_{m,n(t-1)}$ and assume the number of particles in $\mathcal{P}_{m,n(t-1)}$ is $B$.
Let $\mathcal{P}_{m,n(t-1)}^{(i)}$ be the $i^{th}$ particles given both user $m$  and the item $n(t-1)$ at time $t-1$, where $1\le i\le B$. Each particle $\mathcal{P}_{m,n(t-1)}^{(i)}$ has a weight, denoted as $\rho^{(i)}$,  indicating its fitness for the new observed data at time $t$. Note that $\sum_{i=1}^{B}{\rho^{(i)}} = 1$. The fitness of each particle $\mathcal{P}_{m,n(t-1)}^{(i)}$ is defined as the likelihood of the observed data $x_{m,t}$ and $r_{m,t}$. Therefore,
\begin{equation}
  \rho^{(i)} \varpropto p(x_{m,t}, r_{m,t}|\mathcal{P}_{m,n(t-1)}^{(i)}).
\label{eq:computeWeights}
\end{equation}
Further, $y_{m,t}$ is the predicted value of $r_{m,t}$. The distribution of $y_{m,t}$, determined by $\mathbf{p}_m$, $\mathbf{q}_n$, $z_{m,t}$, $\mathbf{\Phi}_k$ , and  $\sigma^2_n$, described in Section~\ref{subsec:dependence-arm}.

Therefore, we can compute $\rho^{(i)}$ as proportional to the density value given $y_{m,t} = r_{m,t}$ and $x_{m,t} = n$.
Thus, we obtain
\begin{equation*}
    \begin{split}
   \rho^{(i)} \varpropto & \sum_{z_{m,t}=1}^{K}\{\mathcal{N}(r_{m,t}|(\mathbf{p}_{m}^\intercal\mathbf{q}_{n},\sigma^2_{n}) \\  &\bullet p(z_{m,t}=k, x_{m,t} = n|\mathcal{P}_{m,n(t-1)}^{(i)})\},
 \end{split}
 \end{equation*}
 where
%\begin{comment}
%\begin{equation*}
%    \begin{split}
%   \rho^{(i)} \varpropto \iint_{z_{m,t},\eta_{j,t-1}}\{\mathcal{N}(\mathbf{r}_{m,t}|(\mathbf{p}_{m}^\intercal\mathbf{q}_{n},\sigma^2_{n}) Mult(z_{m,t} = k|\mathbf{p}_m) \\ Mult(x_{m,t}=n|\Phi_k) Dir(\mathbf{p}_m|\mathbf{\lambda}) Dir(\mathbf{q}_n|\mathbf{\mathbf{\eta}})\mathcal{IG}(\sigma^2_n|\alpha, \beta)\} \\  d\eta_{j,t}\,d\eta_{j,t-1},
% \end{split}
% \end{equation*}
 %\end{comment}
 \begin{equation}
 \begin{split}
   &p(z_{m,t}=k, x_{m,t} = n|\mathcal{P}_{m,n(t-1)}^{(i)}) \\
   &=\iint_{\mathbf{p}_m,\mathbf{\Phi}_k}p(z_{m,t}=k, x_{m,t} = n,\mathbf{p}_m,\mathbf{\Phi}_k|\lambda,\eta)d\mathbf{p}_m,d\mathbf{\Phi}_k \\
   &=\int_{\mathbf{p}_m}Mult(z_{m,t}=k|\mathbf{p}_m)Dir(\mathbf{p}_m|\lambda)d\mathbf{p}_m \\ &\bullet\int_{\mathbf{\Phi}_k}Mult(x_{m,t}=n|\mathbf{\Phi}_k)Dir(\mathbf{\Phi}_k|\eta)d\mathbf{\Phi}_k \\
   &=E(\mathbf{p}_{m,k}|\lambda)\bullet E(\mathbf{\Phi}_{k,n}|\eta).
 \end{split}
 \label{eq:zInfer}
 \end{equation}
 Thus, we have:
 \begin{equation}
   \rho^{(i)} \varpropto \sum_{z_{m,t}=1}^{K}\{\mathcal{N}(\mathbf{r}_{m,t}|(\mathbf{p}_{m}^\intercal\mathbf{q}_{n},\sigma^2_{n})\bullet E(\mathbf{p}_{m,k}|\lambda)\bullet E(\mathbf{\Phi}_{k,n}|\eta)\},
   \label{eq:weight}
 \end{equation}
 where $E(\mathbf{p}_{m,k}|\lambda)$ and $E(\mathbf{\Phi}_{k,n}|\eta)$ represent the conditional expectations of $\mathbf{p}_{m,k}$ and $\mathbf{\Phi}_{k,n}$ given the observed reward $\lambda$ and $\eta$ of $\mathcal{P}_{m,n(t-1)}^{(i)}$ . The expectations can be inferred by $E(\mathbf{p}_{m,k}|\lambda) = \frac{\lambda_{k}}{\sum_{k=1}^{K}{\lambda_{k}}}$ and $ E(\mathbf{\Phi}_{k,n}|\eta) = \frac{\eta_{k,n}}{\sum_{n=1}^{N}{\eta_{k,n}}}.$
 \begin{comment}
 \begin{equation}
   \begin{split}
     E(\mathbf{p}_{m,k}|\lambda) = \frac{\lambda_{k}}{\sum_{k=1}^{K}[\lambda_{k}]},
   \end{split}
   \label{eq:expectP}
   \end{equation}
   and
   \begin{equation}
   \begin{split}
     E(\mathbf{\Phi}_{k,n}|\eta) = \frac{\eta_{k,n}}{\sum_{n=1}^{N}[\eta_{k,n}]},
   \end{split}
   \label{eq:expectPhi}
 \end{equation}
 where $\mathcal{I}(\bullet)$, an indicator function, returns $1$ when the input boolean expression is true, otherwise returns $0$.
 \end{comment}
\begin{comment}
 \begin{equation}
 \begin{split}
   \rho^{(i)} \varpropto  \{ MVST_{(2\cdot\alpha)}[y_{m,t}| \mathbf{p}_m \mathbf{\mu}_{\mathbf{q}_{n(t)}}, \frac{\alpha}{\beta}(\mathbf{I}+{\mathbf{p}_m^{\intercal}}\mathbf{\Sigma}_{\mathbf{q}_{n(t)}}\mathbf{p}_m)] \\ E({\mathbf{\Phi}_{k,n(t)}})  \}
 \end{split}
 \label{eq:weight}
 \end{equation}
 where MVST is multivariate Student distribution with the degrees of freedom $2\cdot\alpha$.
\end{comment}

Before updating any parameters, a re-sampling process is conducted. We replace the particle set $\mathcal{P}_{m,n(t-1)}$ with a new set $\mathcal{P}_{m,n(t)}$, where $\mathcal{P}_{m,n(t)}$ is generated from $\mathcal{P}_{m,n(t-1)}$ using sampling with replacement based on the weights of particles. Then sequential parameter updating is based on $\mathcal{P}_{m,n(t)}.$

 \subsection{Latent State Inference}
 Provided with the new observation $x_{m,t}$ and $r_{m,t}$ at time $t$, the random state $z_{m,t}$ can be one of $K$ topics, and the posterior distribution of $z_{m,t}$ is shown as follows:
 \begin{equation}
   z_{m,t}|x_{m,t},r_{m,t},\mathcal{P}_{m,n(t-1)}^{(i)} \sim Mult(\mathbf{\theta}),
   \label{eq:sampleZ}
 \end{equation}
 where $\mathbf{\theta}\in\mathcal{R}^K$ is the parameter specifying the multinominal distribution. According to Equation~\ref{eq:zInfer}, since
 \begin{equation*}
 p(z_{m,t}|x_{m,t}, r_{m,t},\lambda,\eta) \varpropto p(z_{m,t},x_{m,t}|r_{m,t},\lambda,\eta),
 \end{equation*}
$\theta$ can be computed by $\theta_k \varpropto E(\mathbf{p}_{m,k}|r_{m,t},\lambda)\bullet E(\mathbf{\Phi}_{k,n}|r_{m,t},\eta).$
 Further, $E(\mathbf{p}_{m,k}|r_{m,t},\lambda)$ and $E(\mathbf{\Phi}_{k,n}|r_{m,t},\eta)$ can be obtained as follows,
 \begin{equation}
   \begin{split}
     E(\mathbf{p}_{m,k}|r_{m,t},\lambda) = \frac{\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}}{\sum_{k=1}^{K}[\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}]},
   \end{split}
   \label{eq:expectP}
   \end{equation}
   and
   \begin{equation}
   \begin{split}
     E(\mathbf{\Phi}_{k,n}|r_{m,t},\eta) = \frac{\mathcal{I}(x_{m,t}=n)r_{m,t} + \eta_{k,n}}{\sum_{n=1}^{N}[\mathcal{I}(x_{m,t}=n)r_{m,t} + \eta_{k,n}]},
   \end{split}
   \label{eq:expectPhi}
 \end{equation}
 where $\mathcal{I}(\bullet)$, an indicator function, returns $1$ when the input boolean expression is true, otherwise returns $0$. Specifically, if $r_{m,t}\in\{0,1\}$, the value of $r_{m,t}$ indicates whether $x_{m,t}$ should be included in the preferred item list of the user $m$. If $r_{m,t}\in [0,+\infty)$, the value of $r_{m,t}$ implies how the user $m$ likes the item $x_{m,t}$. Therefore, our solution can effectively handle the non-negative rating score at different scales.
\begin{comment}
  a can be inferred according to Equation~\ref{eq:zInfer}, since
  by recomputed $E(\mathbf{p}_{m,k})$ and $E(\mathbf{\Phi}_{k,n})$.

At time $t-1$, the sufficient statistics for state $z_{m,t-1}$ are the topic-item posterior distribution (i.e., $S^{\mathbf{\Phi}_{k,n}}_{t-1}$) and the user-topic posterior distribution (i.e., $S^{\mathbf{p}_{m,k}}_{t-1}$ ). Provided with the new observation data $x_{m,t}$ and $r_{m,t}$ at time $t$, the sufficient statistics for state $z_{m,t}$ need to be re-computed. We apply the method according to Equation~\ref{eq:calState} to recursively update the sufficient statistics for $z_{m,t}$ based on the new observation and the sufficient statistics at time $t-1$. Let $S^{\mathbf{\Phi}_{k,n}}_{t}$ and $S^{\mathbf{p}_{m,k}}_{t}$ be the new sufficient statistics of state $z_{m,t}$ at time $t$. Then,

 \begin{equation}
   \begin{split}
     & S_{t}^{\mathbf{\Phi}_{k,n}} = \frac{\mathcal{I}(x_{m,t}=n)r_{m,t} + \eta_{k,n}}{\sum_{n=1}^{N}[\mathcal{I}(x_{m,t}=n)r_{m,t} + \eta_{k,n}]}, \\
     & S_{t}^{\mathbf{p}_{m,k}} = \frac{\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}}{\sum_{k=1}^{K}[\mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k}]},
   \end{split}
   \label{eq:stateUpdate}
 \end{equation}
where $\mathcal{I}(\cdot)$ is indicator function. As shown in Equation~\ref{eq:stateUpdate}, both $S_{t}^{\mathbf{\Phi}_{k,n}}$ and $S_{t}^{\mathbf{p}_{m,k}}$ are estimated by the new observation data $x_{m,t}$ and $r_{m,t}$. With the help of the sufficient statistics for the state random variable, $z_{m,t}$ can be obtained shown in Equation~\ref{eq:calState}.

\begin{equation}
 \begin{split}
 P(z_{m,t}|S_{t}^{\mathbf{\Phi}_{k,n}}, S_{t}^{\mathbf{p}_{m,k}}) = S_{t}^{\mathbf{\Phi}_{k,n}} \cdot S_{t}^{\mathbf{p}_{m,k}}
 \end{split}
 \label{eq:calState}
 \end{equation}
\end{comment}
\subsection{Parameter Statistics Inference}
At time $t-1$, the sufficient statistics for the parameter random variables ($\mathbf{q}_n$, ${\sigma^2_n}$, $\mathbf{p}_{m}$,
$\mathbf{\Phi}_{k}$) are ($\mathbf{\mu}_\mathbf{q}$, $\mathbf{\Sigma}_\mathbf{q}$, $\alpha$, $\beta$, $\mathbf{\lambda}$, $\mathbf{\eta}$). Assume $\mathbf{\mu}_\mathbf{q}'$, $\mathbf{\Sigma}_\mathbf{q}'$, $\alpha'$, $\beta'$, $\mathbf{\lambda}'$, $\mathbf{\eta}'$ are the sufficient statistics at time $t$, which are updated on the basis of both the sufficient statistics at time $t-1$ and the new observation data (i.e, $x_{m,t}$ and $r_{m,t}$). The sufficient statistics for parameters are updated as follows:
 \begin{equation}
 \begin{split}
  & \mathbf{\Sigma}_{\mathbf{q}_n}' = (\mathbf{\Sigma}_{\mathbf{q}_n}^{-1} + \mathbf{p}_m\mathbf{p}_m^{\intercal})^{-1} \\
  & \mathbf{\mu}_{\mathbf{q}_n}' = \mathbf{\Sigma}_{\mathbf{q}_n}'(\mathbf{\Sigma}_{\mathbf{q}_n}^{-1}\mathbf{\mu}_{\mathbf{q}_n} + \mathbf{p}_m r_{m,t}) \\
  & \alpha' = \alpha + \frac{1}{2} \\
  & \beta' = \beta + \frac{1}{2}(\mathbf{\mu}_{\mathbf{q}_n}^{\intercal} \mathbf{\Sigma}_{\mathbf{q}_n}^{-1} \mathbf{\mu}_{\mathbf{q}_n} +
  r_{m,t}^{\intercal}r_{m,t} - \mathbf{\mu}_{\mathbf{q}_n}'^{\intercal} \mathbf{\Sigma}_{\mathbf{q}_n}'^{-1} \mathbf{\mu}_{\mathbf{q}_n}') \\
  & \lambda'_{k} = \mathcal{I}(z_{m,t}=k)r_{m,t} + \lambda_{k} \\
  & \eta'_{k,n} = \mathcal{I}(x_{m,t}=n)r_{m,t} + \eta_{k,n}
 \end{split}
 \label{eq:updateParameters}
 \end{equation}

At time t, the sampling process for the parameter random variables ${\sigma^2_n}$, $\mathbf{q}_n$, $\mathbf{p}_{m}$ and
$\mathbf{\Phi}_{k}$ is summarized as below:
\begin{equation}
 \begin{split}
 & \sigma^2_n \sim \mathcal{IG}(\alpha', \beta'), \\
 & \mathbf{q}_n|\sigma^2_n \sim \mathcal{N}(\mathbf{\mu}_{\mathbf{q}_n}', \sigma^2_n\mathbf{\Sigma}_{\mathbf{q}_n}'), \\
 & \mathbf{p}_{m} \sim Dir(\lambda'), \\
 & \mathbf{\Phi}_{k} \sim Dir(\eta').
 \label{eq:sampleParameters}
 \end{split}
\end{equation}

  \subsection{Integration with Policies}\label{sec:policyIntegration}

%of $\mathbf{q}_n$ and $\mathbf{p}_m$ with the hyper parameters $\mathbf{\mu}_{\mathbf{q}_n}$, $\mathbf{\Sigma}_{\mathbf{q}_n}$, $\alpha$, and $\beta.$

%As discussed in Section \ref{subsec:base}, Thompson sampling allocates the pulling chance based on the predicted reward, i.e., the product of $\mathbf{p}_m$ and $\mathbf{q}_n$.
In our interactive collaborative topic regression model, when user $m$ arrives at time $t$, the reward $r_{m,t}$ is unknown since it is not observed until one of arms $x_{m,t}$ is pulled. Without observed $x_{m,t}$ and $r_{m,t}$, the particle re-sampling, latent state inference, and parameter statistics inference for time $t$ cannot be conducted. Therefore, we utilize the latent vectors $\mathbf{p}_m$ and $\mathbf{q}_n$, sampled from their corresponding posterior distributions by Equation~\ref{eq:sampleParameters} at time $t-1$, to predict the reward for every arm. In this section, two policies for interactive collaborative filtering, based on Thompson sampling and UCB (\underline{U}pper \underline{C}onfidence \underline{B}ound), are integrated with our model.

In our model, given the user $m$, every item has $B$ independent particles. Each particle $i$ contains its latent variables and parameters, and produces an independent reward prediction $r_{m,t}^{(i)}.$

Specifically, according to Thompson sampling discussed in Section~\ref{subsec:base}, we predict the reward of pulling arm $n$ with the average value of rewards from $B$ particles. %  as the final reward if pulling arm $n$.%, i.e., $$\bar{r}_{m,n} = \frac{1}{B}\sum_{i=1}^{B}{\mathbf{p}_m^{(i)\intercal}\mathbf{q}_n^{(i)}}.$$
The policy based on Thompson sampling selects an arm $n(t)$ based on the following equation,
\begin{equation}
  n(t) =\arg\max_{n}{(\bar{r}_{m,n})},
  \label{eq:selectArmTS}
\end{equation}
where $\bar{r}_{m,n}$ denotes the average reward, i.e., $$\bar{r}_{m,n} = \frac{1}{B}\sum_{i=1}^{B}{\mathbf{p}_m^{(i)\intercal}\mathbf{q}_n^{(i)}}.$$

Moreover, the UCB policy selects an arms based on the upper bound of the predicted reward. Assuming that $$r_{m,t}^{(i)}
\sim \mathcal{N}(\mathbf{p}_m^{(i)\intercal}\mathbf{q}_n^{(i)},{\sigma^{(i)2}}),$$ the UCB based policy is developed by the mean and variance of predicted reward, i.e.,
\begin{equation}
  n(t) = \arg\max_{n}{(\bar{r}_{m,n} + \gamma\sqrt{\nu})},
\label{eq:selectArmUCB}
\end{equation}
where $\gamma \ge 0$ is a predefined threshold, and the variance is expressed as,
$$\nu = \frac{1}{B}\sum_{i}^{B}{\sigma^{(i)2}}.$$
%Besides $\bar{r}_{m,n}$, the variance ,therefore, the mean of the reward is expressed as $\bar{r}_{m,t} $

\begin{comment}
\textbf{Thompson Sampling.}
Furthermore, given the user $m$, every item has $B$ independent particles. Each particle $i$ produces an independent reward prediction $r_{m,t}^{(i)} = \mathbf{p}_m^{(i)\intercal}\mathbf{q}_n^{(i)}$. We take the average predicted reward as the final reward. Thompson sampling selects the arm $n(t)$ based on the following equation,

\begin{equation}
  n(t) =\arg\max_{n}{(\frac{1}{B}\sum_{i=1}^{B}{\mathbf{p}_m^{(i)\intercal}\mathbf{q}_n^{(i)}})}.
  \label{eq:selectArm}
\end{equation}

Within a single particle of an item $n(t-1)$ at time $t-1$, the distribution of $\mathbf{q}_{n(t-1)}$ can be derived by
   \begin{equation}
        \mathbf{q}_{n(t-1)} \thicksim \mathcal{N}(\mathbf{\mu}_{\mathbf{q}_{n(t-1)}}, \sigma^2_{n(t-1)}\mathbf{\Sigma}_{\mathbf{q}_{n(t-1)}}),
   \end{equation}
   where
   \begin{equation}
     \begin{split}
       &\mathbf{\mu}_{\mathbf{q}_{n(t)}} = (\mathbf{\Sigma}_{\mathbf{q}_{n(t-1)}}^{-1} + \mathbf{p}_m^{\intercal}\mathbf{p}_m)^{-1}(\mathbf{\Sigma}_{\mathbf{q}_{n(t-1)}}^{-1}\mathbf{\mu}_{\mathbf{q}_{n(t-1)}} + \mathbf{p}_m^{\intercal}r_{m,t}) \\
       &\mathbf{\Sigma}_{\mathbf{q}_{n(t)}} = (\mathbf{\Sigma}_{\mathbf{q}_{n(t-1)}}^{-1} + \mathbf{p}_m^{\intercal}\mathbf{p}_m)^{-1}
     \end{split}
   \end{equation}
   Let $\mathbf{q}^{(i)}_{n(t-1)}$, $\mathbf{\mu}^{(i)}_{\mathbf{q}_{n(t-1)}}$, ${\sigma}_{n(t-1)}^{2(i)}$, and $\mathbf{\Sigma}^{(i)}_{\mathbf{q}_{n(t-1)}}$ be the random variables in the $i^{(th)}$ particle. We use the mean of $\mathbf{q}_{n(t-1),t-1}$,, denoted as $\bar{\mathbf{q}}_{n(t-1),t-1}$, to infer the decision in the bandit algorithm. Therefore,
   \begin{equation}
    \label{eq:posterMean}
     \bar{\mathbf{q}}_{n(t-1)} \thicksim \mathcal{N}(\mathbf{\bar{\mu}}_{\mathbf{q}_{n(t-1)}},\mathbf{\bar{\Sigma}}_{\mathbf{q}_{n(t-1)}}),
   \end{equation}
   where
   \begin{equation}
     \begin{split}
       &\mathbf{\bar{\mu}}_{\mathbf{q}_{n(t-1)}} = \frac{1}{p}\sum_{i=1}^{p}{\mathbf{\mu}^{(i)}_{\mathbf{q}_{n(t-1)}}}, \\
       &\mathbf{\bar{\Sigma}}_{\mathbf{q}_{n(t-1)}}= \frac{1}{p^2}\sum_{i=1}^{p}{{\sigma}_{n(t-1)}^{2(i)}\mathbf{\bar{\Sigma}}_{\mathbf{q}_{n(t-1)}}}.
     \end{split}
   \end{equation}

\noindent \ \ \ \ By virtual of Equation~\ref{eq:posterMean}, Thompson sampling can address the bandit problem as mentioned in Section~\ref{subsec:base}. Specifically, Thompson sampling draws $\mathbf{q}_{n(t),t}$ from Equation~\ref{eq:posterMean} and then predicts the rating for each item with $\mathbf{p}_{m,t}$. The item with maximum predicted rating is selected to recommend. While UCB selects an item with a maximum score, where the score is defined as a combination of the expectation of $y_{m,t}$ and its standard deviation, i.e.,
 \begin{equation*}
   E(y_{m,t}|\mathbf{p}_{m,t}) + \lambda\sqrt{Var(y_{m,t}|\mathbf{p}_{m,t})},
 \end{equation*} where $\lambda$ is predefined parameter, $E(y_{m,t}|\mathbf{p}_{m,t})$ and $Var(y_{m,t}|\mathbf{p}_{m,t})$ are computed by
 %It is straightforward  to compute the expectation by
 $$E(y_{m,t}|\mathbf{p}_{m,t}) = \mathbf{p}_{m,t}^\intercal\mathbf{q}_{n(t)}.$$
 %However,
 $$Var(y_{m,t}|\mathbf{p}_{m,t})= \mathbf{p}_{m,t}^\intercal\mathbf{\bar{\Sigma}}^{-1}_{\mathbf{q}_{n(t)}}\mathbf{p}_{m,t} + \frac{1}{p^2}\sum_{i=1}^{p}{\sigma^2_{n(t)}}.$$
\end{comment}
\subsection{Algorithm}
Putting all the aforementioned inference together, an algorithm based on the interactive collaborative topic regression model is provided below.

Online inference for the interactive collaborative filtering problem starts with $\text{MAIN}$ procedure, as presented in Algorithm~\ref{alg:ictr}. As user $m$ arrives at time $t$, the $\text{EVAL}$ procedure computes a score for each arm, where we define the score as the average reward. The arm with the highest score is selected to pull. After receiving a reward by pulling an arm, the new feedback is used to update the ICTR model by the $\text{UPDATE}$ procedure. Especially in the $\text{UPDATE}$ procedure, we use the $resample$-$propagate$ strategy in particle learning~\cite{carvalho2010particle} rather than the $propagate$-$resample$ strategy in particle filtering~\cite{djuric2003particle}. With the $resample$-$propagate$ strategy, the particles are re-sampled by taking $\rho^{(i)}$ as the $i^{th}$ particle's weight, where the $\rho^{(i)}$ indicates the fitness for the observation at time $t$ given the particle at time $t-1$. The $resample$-$propagate$ strategy is considered as an optimal and fully adapted strategy, avoiding an importance sampling step.

  \begin{algorithm}[!htp]
    \caption{The algorithm for interactive collaborative topic regression model (\texttt{ICTR})}
     \label{alg:ictr}
    \begin{algorithmic}[1]
        \Procedure{main}{$B$}\Comment{main entry}
            \State {Initialize $B$ particles, i.e., $\mathcal{P}_{m,n(0)}^{(1)}...\mathcal{P}_{m,n(0)}^{(B)}$.}
            %\State {Initialize each user with $B$ particles.}
            %\State {Initialize each topic with $B$ particles.}
            \For {$t\gets 1, T$}
            \State{User $m$ arrives for item recommendation.}
            %\State {Get the latent vector $\mathbf{p}_{m}$ for current user $m$.}
            \State {$n(t) = \arg\max_{n=1,N}{\text{EVAL}(m,n)}$}\Comment{by Eq.~\ref{eq:selectArmTS} or Eq.~\ref{eq:selectArmUCB}.}
            \State {Receive $r_{m,t}$ by rating item $n(t)$.}
            \State {\text{UPDATE}($m$, $n(t)$, $r_{m,t}$). }
            \EndFor
        \EndProcedure
        \Statex{}
        \Procedure {eval}{$m$, $n$}\Comment{get a rating score for item $n$, given user $m$.}
            \For {$i\gets 1, B$}\Comment{Iterate on each particle.}
            \State{Get the user latent vector $\mathbf{p}_m^{(i)}$.}
            \State{Get the item latent vector $\mathbf{q}_n^{(i)}$.}
            \State{Predict $i^{th}$ reward $r_{m,t}^{(i)}$.}
            \EndFor
            \State{Compute the average reward as the final reward $r_{m,t}$.}
            \State \textbf{return} {the score.}
        \EndProcedure
        \Statex{}
        \Procedure {update}{$m$, $n(t)$, $r_{m,t}$}\Comment{update the inference.}
            \For {$i\gets 1, B$}\Comment{Compute weights for each particle.}
                \State {Compute weight $\rho^{(i)}$ of particle $\mathcal{P}_{m,n(t)}^{(i)}$ by Eq.~\ref{eq:computeWeights}.}
            \EndFor
            \State {Re-sample $\mathcal{P'}_{m,n(t)}$ from $\mathcal{P}_{m,n(t)}$ according to the weights $\rho^{(i)}$s.}
            \For {$i\gets 1, B$}\Comment{Update statistics for each particle.}
                \State {Update the sufficient statistics for $z_{m,t}$ by Eq.~\ref{eq:expectP} and~\ref{eq:expectPhi}.}
                \State {Sample $z_{m,t}$ according to Eq.~\ref{eq:sampleZ}.}
                \State {Update the statistics for $\mathbf{q}_n$, ${\sigma^2_n}$, $\mathbf{p}_{m}$,
$\mathbf{\Phi}_{k}$ by Eq.~\ref{eq:updateParameters}.}
                \State {Sample $\mathbf{q}_n$, ${\sigma^2_n}$, $\mathbf{p}_{m}$,
$\mathbf{\Phi}_{k}$ according to Eq.~\ref{eq:sampleParameters}.}
            \EndFor
        \EndProcedure
    \end{algorithmic}
  \end{algorithm}


In addition, existing algorithms~\cite{zhao2013interactive,kawale2015efficient} consider all the arms independently, while our model takes the clusters of arms into account by learning the topic-related random variables (e.g., $\Phi_k$). Those topic related random variables are shared among all the arms.

==> relatedwork-bak.tex <==
\section{Related Work} \label{sec:relatedwork}
In this paper, we come up with an interactive collaborative topic regression model recommending an item to the user in an interactive way by leveraging multi-armed bandit algorithms with dependent arms. Also, a sequential online inference method is proposed to learn the latent unknown parameters and infer the latent states. In this section, we highly review the existing works that related to our approach.

\subsection{Recommendation by Matrix Factorization}
%% cf
The collaborative filtering (CF) methods play a central role to recommenders system. Without need for extra information about either items or users, CF recommends items to a target user based on patterns of ratings. There are two primary categories of CF technologies: The memory-based methods~\cite{sarwar2001item, herlocker1999algorithmic} focus on making the recommendation by modeling the relationships between similar items or users, while the model-based methods~\cite{salakhutdinov2007probabilistic, salakhutdinov2008bayesian, agarwal2009regression, ungar1998clustering} provide an alternative approach by developing a model of user ratings. For instance, latent factor models provides better recommendation by projecting both users and items into the a shared low-dimension latent factor space.
%% mf challenge cold-start problem online setting

Among the latent factor models, the matrix factorization~\cite{koren2009matrix} technologies have gained popularity recently due to Netflix Prize and other recommendation competitions. Probabilistic Matrix Factorization (PMF)~\cite{salakhutdinov2007probabilistic} proposes a probabilistic linear algorithm to model observed ratings with Gaussian observation noise. Bayesian Probabilistic Matrix Factorization (BPMF)~\cite{salakhutdinov2008bayesian} presents a fully Bayesian treatment of the Probabilistic Matrix Factorization (PMF) model. Notwithstanding the MF-based methods have been successfully applied into various recommender systems, one of the key challenges faced by these methods is to how to effectively recommend when a new user/item arrives in the recommender system, also referred as cold-start problem. Interactive Collaborative Filtering (ICF)~\cite{zhao2013interactive} studies collaborative filtering in an interactive setting by integrating PMF framework and leveraging multi-armed bandit algorithms to resolve the cold-start problem only considering the user side. Another challenge is to sequentially recommend items to the target user in an online setting and instantly adapt the up-to-date feedback to refine the recommendation predictions. Many real world applications including online personalized advertising and news recommendation try to continuously maximize the consumers' satisfaction in the long run~\cite{zeng2016online}. Particle Thompson Sampling for MF~\cite{kawale2015efficient} studies Rao-Blackwellized particle based on Thompson sampling framework for online matrix factorization.

\subsection{Matrix Factorization with Probabilistic Topic Models}
Recently, several attempts~\cite{wang2011collaborative,purushotham2012collaborative} have been made by researchers to combine collaborative filtering based on matrix factorization and topic modeling~\cite{blei2003latent}. The central idea behind these methods is to leverage topic modeling to capture items content information in latent topic space and focus on combining the merits of both traditional collaborative filtering and probabilistic topic modeling approaches. Different from the above studies, topic modeling is utilized to soft cluster items as topics based on local matrix factorization~\cite{wangbayesian}.

\subsection{Multi-armed Bandit Algorithms}
The recommender systems are required to balance the tradeoff between \textit{exploration} and \textit{exploitation}: maximizing user satisfaction using the history records, while gathering new information for improving recommendation predictions between user preference and items. This dilemma has been well dealt with by a series of multi-armed bandit algorithms including $\epsilon$-greedy algorithm~\cite{tokic2010adaptive}, upper confidence bound (UCB)~\cite{auer2002using}, EXP3~\cite{auer2002nonstochastic} and Thompson sampling~\cite{chapelle2011empirical}.

%$\epsilon$-greedy algorithm is a simple bandit policy by choosing the best arm (the highest average reward) with probability $1-\epsilon$ and randomly
%playing an arm with probability $\epsilon$. UCB policy leverages upper confidence bounds for \textit{exploration} and \textit{exploitation} dilemma and achieves a regret bound of $O(n\sqrt{T})$~\cite{auer2002using}. Thompson sampling~\cite{chapelle2011empirical} is a more flexible algorithm by randomly allocating the pulling chance according to the probability that an arm provides the highest expected reward. In~\cite{zhao2013interactive}, Thompson sampling is applied to model their interaction by considering the distribution of latent feature vectors of both the user and the item.

% contextual multi-armed bandit
 Online personal advertising~\cite{anagnostopoulos2007just,tang2015personalized,zeng2016online} and news article recommendation~\cite{li2010contextual,tang2015personalized,zeng2016online} have successfully engaged contextual multi-armed bandit algorithms to address the cold-start problem, where the contextual features including the user information (e.g., demographic information and behavior targeting features) and item description (e.g., category and type information), are utilized for arm selection.
% multi-armed bandit with dependent arms

However, most of the prior bandit problems focuses on independent arms. A delicate framework~\cite{pandey2007multi} is developed to study the bandit problems with dependent arms, where the dependencies are in the form of a generative model on clusters of arms.
\subsection{Sequential Online Inference}
Sequential online inference algorithm is well developed to learn the latent unknown parameters and infer the latent states in our model. Sequential monte carlo sampling~\cite{halton1962sequential, doucet2001introduction} and particle learning~\cite{carvalho2010particle} are both popular sequential learning methods.

Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution to address the filtering problem~\cite{doucet2000sequential}. By using these methods, discrete time dynamic models typically both nonlinear and non-Gaussian are allowed inference for full posterior distributions.
Particle learning (PL) provides state filtering, sequential parameter learning and smoothing in a large class of state space models~\cite{carvalho2010particle}. Particle learning is an approach approximating the sequence of filtering and smoothing distributions in light of parameter uncertainty for a wide class of state space models.  The central idea behind PL is the creation of a particle algorithm that directly samples from the particle approximation to the joint posterior distribution of states and conditional sufficient statistics for fixed parameters in a fully-adapted re-sample propagate framework.





==> relatedwork1.tex <==
\section{Related Work} \label{sec:relatedwork}
%In this paper, we introduce an interactive collaborative topic regression model that utilizes multi-armed bandit algorithms with dependent arms for the item recommendations to the target user.
%A sequential online inference method is proposed to learn the latent parameters and infer the latent states.
In this section, we review the existing work related to our approach.
\subsection{Collaborative Filtering}
%% cf
Collaborative filtering (CF)~\cite{linden2003amazon} methods play a key role in recommender systems
%. Without need for extra information about either items or users, CF
that recommend items to a target user only based on users' historical ratings of items. There are two primary categories of CF technologies. The memory-based methods~\cite{sarwar2001item, herlocker1999algorithmic} focus on making a recommendation by computing the similarity between items or users, while the model-based methods~\cite{salakhutdinov2007probabilistic, salakhutdinov2008bayesian, agarwal2009regression, ungar1998clustering} develop models using data mining and machine learning techniques to find patterns based on ratings. In addition, it handles the sparsity better than memory-based methods such as matrix factorization ~\cite{koren2009matrix} (MF) technologies, which project both users and items into a shared low dimension latent factor space.
%. For instance, latent factor models provide better recommendation by projecting both users and items into a shared low-dimension late\nt factor space.
%% mf challenge cold-start problem online setting

The matrix factorization technologies gained popularity due to the Netflix Prize and other recommendation competitions.
A significant  variety of MF-based methods are proposed.
Probabilistic Matrix Factorization (PMF)~\cite{salakhutdinov2007probabilistic} models the ratings as products of users' and items' latent features and adds Gaussian observation noise.
PMF can scale linearly with number of observations and perform well on very sparse and imbalanced data.
%A fully Bayesian treatment of PMF (BPMF)~\cite{salakhutdinov2008bayesian} present
Bayesian Probabilistic Matrix Factorization (BPMF)~\cite{salakhutdinov2008bayesian} presents a fully Bayesian treatment of the PMF model with priors controlling model complexity automatically.
%Notwithstanding the fact that MF-based methods have been successfully applied into various recommender systems,
However, one of the key challenges existing in the aforementioned methods is effective recommendation for users or items that have not yet gathered sufficient rating information.
This challenge is usually referred to as a cold-start problem.
Interactive Collaborative Filtering (ICF)~\cite{zhao2013interactive} tackles the cold-start problem in an interactive setting by integrating PMF framework and multi-armed bandit algorithms only considering the user side. Particle Thompson Sampling for MF [15] studies Rao-Blackwellized particle based on Thompson sampling framework for online matrix factorization.
Studies~\cite{zeng2016online, kawale2015efficient} undertake the online personalized advertising and news article recommendation tasks~\cite{anagnostopoulos2007just,tang2015personalized,li2010contextual} in an online setting where the model instantly adopts up-to-date feedback to refine the recommendation predictions.
The incorporation of the up-to-date feedback is implemented by sequential online inference techniques.
Moreover, they used contextual multi-armed bandit algorithms to address the cold-start problem, by selecting arms based on the contextual features of the users' information and items' description.

\subsection{Sequential Online Inference \& Multi-armed Bandit Algorithms}
Sequential online inference techniques are well developed for learning the latent parameters and inferring the latent states.
One such technique is sequential Monte Carlo sampling~\cite{halton1962sequential, doucet2001introduction, carvalho2010particle}.
Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution for addressing the filtering problem~\cite{doucet2000sequential}. By using these methods, discrete time dynamic models, typically both nonlinear and non-Gaussian, are allowed to inference for full posterior distributions.
%
Multi-armed bandit algorithms are designed to deal with the demand of balancing the tradeoff between \textit{exploration} and \textit{exploitation} in a recommender system that requires maximizing user satisfaction using history records, while gathering new information for improving recommendation predictions between user preference and items. Classical multi-armed bandit algorithms include $\epsilon$-greedy algorithm~\cite{tokic2010adaptive}, upper confidence bound (UCB)~\cite{auer2002using}, EXP3~\cite{auer2002nonstochastic} and Thompson sampling~\cite{chapelle2011empirical}.

\begin{comment}
\subsection{Sequential Online Inference}
Sequential online inference algorithm is well developed for learning the latent unknown parameters and inferring the latent states in our model. Sequential monte carlo sampling~\cite{halton1962sequential, doucet2001introduction} and particle learning~\cite{carvalho2010particle} are both popular sequential learning methods.

Sequential Monte Carlo (SMC) methods, also known as particle filters, are a set of simulation-based methods for computing the posterior distribution for addressing the filtering problem~\cite{doucet2000sequential}.
Usage of these methods allows inference of the full posterior distributions for the discrete time dynamic models both nonlinear and non-Gaussian.

Particle learning (PL) provides state filtering, sequential parameter learning and smoothing in a large class of state space models~\cite{carvalho2010particle}.
Particle learning is an approach approximating the sequence of filtering and smoothing distributions with parameter uncertainty for a wide class of state space models.
The central idea behind PL is the creation of a particle algorithm that directly samples from the particle approximation to the joint posterior distribution of states and generates sufficient statistics for fixed parameters in a fully-adapted re-sample propagation framework.
\end{comment}

%Another challenge is to sequentially recommend items to the target user in an online setting and instantly adopt the up-to-date feedback to refine the recommendation predictions. Many real world applications including online personalized advertising and news recommendation continuously maximize the consumers' satisfaction in the long run~\cite{zeng2016online}. Particle Thompson Sampling for MF~\cite{kawale2015efficient} studies Rao-Blackwellized particle based on Thompson sampling framework for online matrix factorization.

%\subsection{Matrix Factorization with Probabilistic Topic Models}
Recently, several attempts~\cite{wang2011collaborative,purushotham2012collaborative,wangbayesian} have been made by researchers to model the dependence between items utilizing topic modeling~\cite{blei2003latent} in MF-based Collaborative filtering.
The core idea behind these methods is to apply topic modeling on items' content information to softly cluster items and share the feedback among clusters.
%focus on combining the merits of both traditional collaborative filtering and probabilistic topic modeling approaches.
%Different from the above studies, topic modeling is utilized to soft cluster items as topics based on local matrix factorization~\cite{wangbayesian}.
Different from the above studies, our method not only needs no items' content information to model the dependence between items, but also recommend items in MF-based collaborative filtering with an online setting.

\begin{comment}
\subsection{Multi-armed Bandit Algorithms}
The recommender systems are required to balance the tradeoff between \textit{exploration} and \textit{exploitation}: maximizing user satisfaction using the history records, while gathering new information for improving recommendation predictions between user preference and items. This dilemma has been well dealt with by a series of multi-armed bandit algorithms including $\epsilon$-greedy algorithm~\cite{tokic2010adaptive}, upper confidence bound (UCB)~\cite{auer2002using}, EXP3~\cite{auer2002nonstochastic} and Thompson sampling~\cite{chapelle2011empirical}.


$\epsilon$-greedy algorithm is a simple bandit policy by choosing the best arm (the highest average reward) with probability $1-\epsilon$ and randomly
playing an arm with probability $\epsilon$. UCB policy leverages upper confidence bounds for \textit{exploration} and \textit{exploitation} dilemma and achieves a regret bound of $O(n\sqrt{T})$~\cite{auer2002using}. Thompson sampling~\cite{chapelle2011empirical} is a more flexible algorithmthat  randomly allocates the pulling chance according to the probability that an arm provides the highest expected reward. In~\cite{zhao2013interactive}, Thompson sampling is applied to modelling their interaction by considering the distribution of latent feature vectors of both the user and the item.

% contextual multi-armed bandit
 Online personal advertising~\cite{anagnostopoulos2007just,tang2015personalized,zeng2016online} and news article recommendation~\cite{li2010contextual,tang2015personalized,zeng2016online} have successfully engaged contextual multi-armed bandit algorithms to address the cold-start problem, where the contextual features include the user information (e.g., demographic information and behavior targeting features) and item description (e.g., category and type information), are utilized for arm selection.
% multi-armed bandit with dependent arms

However, most of the prior bandit problems focuses on independent arms. A delicate framework~\cite{pandey2007multi} is developed to study the bandit problems with dependent arms, where the dependencies are in the form of a generative model on clusters of arms.
\end{comment}





